Estimation-Action-Reflection: Towards Deep Interaction Between Conversational and Recommender Systems

Recommender systems are embracing conversational technologies to obtain user preferences dynamically, and to overcome inherent limitations of their static models. A successful Conversational Recommender System (CRS) requires proper handling of interactions between conversation and recommendation. We argue that three fundamental problems need to be solved: 1) what questions to ask regarding item attributes, 2) when to recommend items, and 3) how to adapt to the users' online feedback. To the best of our knowledge, there lacks a unified framework that addresses these problems. In this work, we fill this missing interaction framework gap by proposing a new CRS framework named Estimation-Action-Reflection, or EAR, which consists of three stages to better converse with users. (1) Estimation, which builds predictive models to estimate user preference on both items and item attributes; (2) Action, which learns a dialogue policy to determine whether to ask attributes or recommend items, based on Estimation stage and conversation history; and (3) Reflection, which updates the recommender model when a user rejects the recommendations made by the Action stage. We present two conversation scenarios on binary and enumerated questions, and conduct extensive experiments on two datasets from Yelp and LastFM, for each scenario, respectively. Our experiments demonstrate significant improvements over the state-of-the-art method CRM [32], corresponding to fewer conversation turns and a higher level of recommendation hits.

==> Intro_BAK.tex <==

%% Min: to edit and re-write the intro
With recommendation systems and dialogue agents becoming standard fixtures in workflows, there is an unprecedented opportunity to define how these two technologies can be interwoven.  We envision this intersection as the rise of the {\it conversational recommendation system} (CRS), a system role that allows a dialog agent to recommend items to a user with a naturalistic, dialogic setting, sensitive to the particular mannerisms of human dialog.  We define a basic framework for this scenario, analogous to an exploration–exploitation tradeoff, that allows the system perform two actions: 1) to pose questions (explore) to obtain preferences from the user as well as 2) recommend items (exploit) to the user.

Recommendation systems traditionally use a static user profile, inferred from a user's historical actions, to recommend items for consumption.  While of great success, this approach's key weakness is that it computes an implicit model of the user's need.  What if the agent can interrogate the user directly?  With the advent of dialogue agents, this possibility is more naturally realized through dialog with the user.  

% Could put more emphasis on the difficulty of doing this.
Our CRS framework weaves dialog with recommendation at a fine-grained level, achieving deep interaction.  When the system is uncertain, it queries the user for her preferences to achieve maximal certainty towards relevant recommendations.  When the system reaches sufficient confidence, it recommends items.  This interaction is dynamic, meaning it can switch between both modes in online interactions on a per-turn basis, mimicking human behavior in dialog.  Our proposed {\it Estimation-Action-Reflection} (EAR) asks three key questions in implementing this framework: 1) what questions to ask regarding item attributes, 2) when to recommend items, and 3) how to adapt to the user's feedback.  

We develop our basic EAR framework by describing items as having a set of binary attributes, in which the system can query the user's preference on  selected attribute.  We then further develop the notion of enumerated attributes, where an attribute can take on an enumerated set of values.  Our extended EAR model optimally queries for such enumerated attributes.  We show how a large attribute set can be reduced to a compact set of enumerated attributes to make relevant recommendation efficient.

DONE.


\begin{itemize}
    \item Static has problems
    \item Ask Directly
    \item Semi-formal problem framework.  2 Actions: binary ask or recommend.
    \item Complication: can ask enumerated when attributes are many
\end{itemize}

%% Min: end


%%%Wenqiang initial intro
% Too technical at the very beginning. Too much terminology gives a sharp starting of a paper.
% for example: Min cannot understand what the "induce user preference"
% At the beginning of the introduction, the terminology must be correct. Otherwise, it will confuse the reader.
The rapidly developed conversation systems (CS) bring revolutions to this imprecise and incorrect preference estimation problem. Equipped with CS, a \textbf{conversational recommendation system} (CRS) is able to explicitly ask, verify and even induce users preference through natural languages in an interactive way. For example, in Figure XXX right, a CRS can ask questions like \emph{would you like some electronic devices?} if it is not sure the user's current preferences. This type of interaction is different from multi-armed bandit learning \cite{LinUCB}, an existing interactive recommendation framework which captures user dynamic preference. It keeps recommending items to users and inferring their implicit preferences by observing their actions like clicking, buying and skipping items. However, the preference inferred is also implicit which still suffers from the imprecise and incorrect problem. As a key difference, a CRS does not only infer implicit preferences through user action, but also explicitly consult with them about their preference by asking facets (a.k.a. aspects) of items using natural languages.


We consider a realistic conversational recommendation scenario: a CRS interact with a user by asking features and attempting to recommend items multiple times till he/she chooses satisfying items or leaves the current session. This is more sophisticated
% Wenqiang: sophisticated indicates something incremental.
% wording: fundamentally different.
than existing settings \citet{Sun:2018:CRS:3209978.3210002, zhang2018towards} where a system is designed to make a recommendation at the end of each session. In our scenario, a CRS need a more comprehensive strategy. It may act conservatively, keep asking features until its confidence towards user preference is high enough. Alternatively, it can also take chances to recommend items when achieving a certain level of confidence and adjust its strategy once a recommendation is rejected. The key challenge is to make full use of every single turn to get a satisfactory recommendation within fewer turns because users have limited patience.

As a combination of a RS and a CS, a CRS raises new challenges for both sides. Compared to traditional static recommendation setting, real-time user feedbacks from the CS are available. Such feedbacks indicate user preference explicitly (e.g., telling a facet that he/she prefers) or implicitly (e.g., rejecting a recommendation). How to leverage on both explicit and implicit indications in a CRS still remains to be an open question. On the conversation side, a CRS is also different from traditional task-oriented dialogue systems (cite) which enumeratively check all facets of items with users and demonstrate qualified items to them. A CRS's choice of dialogue action need to consider the estimation of the RS component, with the aim of achieving a successful recommendation within less turns. For example, a CRS does not need to waste a turn to ask a question like \emph{do you like some books?} if the RS thinks he scarcely possible to buy books. Note that we consider a realistic conversational recommendation scenario where a CRS can ask features and recommend items multiple times. This is more sophisticated and challenging than existing settings \citet{Sun:2018:CRS:3209978.3210002, zhang2018towards} where a system is designed to make a recommendation only at the end of each session. This sophisticated scenario  makes the problem even more challenging as a CRS need to make more complicated decisions.

Although some progress has been made along the line of conversational or interactive recommendation, existing research is not focused on the interaction between CS and RS, far from being usable for real-world scenarios. Particularly, state-of-the-art CRS methods either ignore the strategy for when to recommend~\cite{zhang2018towards,nips18/DeepConv} or only consider single-round conversation that recommends items once~\cite{christakopoulou2018q,Sun:2018:CRS:3209978.3210002}. 
To our knowledge, there lacks a unified framework that can jointly solve the three problems well.

Towards the goal of building an effective CRS suitable for practical use, we focus on the extensive interaction between the CS and RS. We propose a new solution named \textit{Estimation-Action-Reflection} (EAR), which consists of three stages: 
%\begin{enumerate}[leftmargin=*]
(a) Estimation, which builds predictive models offline to estimate user preference on items and item attributes. 
%It provides support for the conversational strategy that determines whether to ask/recommend and what questions to ask about item attributes. 
We train a factorization machine~\cite{rendle2010factorization}~(FM) using user profiles and item attributes as input features, with two novelties in: 1) jointly optimizing FM on the two tasks of item prediction and attribute prediction, and 2) revising the training process on conversation data to ensure the model works well with online user feedback on attributes. 
(b) Action, which learns 
the conversational strategy that determines whether to ask or recommend, and what attribute questions to ask. We train a policy network with reinforcement learning, optimizing the reward of short turns and successful recommendations based on FM's estimation of the preferred items, attributes, and dialogue histories. 
(c) Reflection, which adapts the CRS with user online feedback. Specifically, when a user rejects the recommended items, we construct new training triplets by treating the items as negatives and update FM in an online manner.  

%%%%wenqiang initial tro end


%% Wenqiang editted by yisong
\textbf{Static has problems:}
Recommendation systems (RS) have proven to be successful in online services, e.g., suggesting products in e-commerce platforms. Such systems learn users' implicit preferences towards items based on their historical actions (e.g., buying a product). However, the offline static recommender systems have intrinsic limitation. As a usual case, the short of historic data may lead offline learned preference to be imprecise. Even if the historic data is abundant, the learned preference may not conform with user's current need, the estimation for user's preference can be imprecise as the user intention is dynamic and shifting as per recommendation session. An example is illustrated in Figure (XXX left), in a e-commerce platform, a user usually buys four categories of products: electronic devices and clothes. When he visit the platform again, a well-trained RS is supposed to recommend all the two types of products regardless of what the user want to buy at this time, resulting in a imprecise recommendation. In the case where insufficient actions have been recorded for a user, the recommendation will be more imprecise or even incorrect.

\textbf{Ask Directly:}
%Candidate 1
%With the recent improvement of conversational systems including Siri, Cortana, internet users are enjoying the convenience to communicate directly with such systems to accomplish their daily needs or find answer for a question. It is natural to ask, is it possible to conduct the recommendation procedure in an conversational way?
%Candidate 2, Yisong preferred.
In a traditional recommendation scenario, a user can only passively perceive the recommended items from the system and cannot explicitly tell the system her need. In the meantime, the system has difficulty to predict user's current need as user cannot inform it. Therefore there is a gap between the system and user, which can be addressed in a conversational way.

\textbf{Semi-formal problem framework}
To formalize this as a researchable problem, we devise two types of action for the system: raising a question and make recommendation. By raising a question, the user can respond her preference for an attribute to help the system narrow the candidate items. By making recommendation, the user will accept when the desired items is within the recommendation list. We will have a detailed definition in Section 2.


----------------


==> ear-arxiv-new/Conclusion.tex <==
% \vspace{-5pt}
\section{Conclusion and Future Work}
In this work, we redefine the conversational recommendation task where the RC and CC closely support each other so as to achieve the goal of accurate recommendation in fewer turns. 
%We consider a multi-round conversational recommendation scenario 
We decompose the task into three key problems, namely, what to ask, when to recommend, and how to adapt with user feedback. We then propose EAR -- a new three-stage solution accounting for the three problems in a unified framework. For each stage, we design our method to carefully account for the interactions between RC and CC. Through extensive experiments on two datasets, we justify the effectiveness of EAR, providing additional insights into the conversational strategy and online updates. 
%Such problem 

%We implement such interaction within three stages, namely \emph{estimation}, \emph{action} and \emph{reflection}. 

%In this work, we consider multi-round scenario for conversational recommendation system, which is a more realistic and sophisticated setting than existing works. This raises new challenges for both recommendation systems and conversation systems. To address them, we hypothesize the key locates on the interaction between the conversation component and the recommendation component. This lead to our EAR system which achieves such collaborations in three stage, namely \emph{estimation}, \emph{action} and \emph{reflection}. In our empirical experiment on two datasets, EAR beats strong baselines, validating the efficacy of our three-stage strategy.

%data, online experiment sourunding
%updating policy
%more effective online updating strategy
%language understanding
%simulate dislike

Our work represents the first step towards exploring how the CC and RC can collaborate closely to provide quality recommendation service in this multi-round scenario. Naturally, there are thus a few loose ends for further investigation, especially with respect to incorporating user feedback. 
% For example, when the user rejects the asked attribute, our current EAR updates actions by only refreshing the state vector that encodes the dialogue history. 
In the future, we will consider refreshing the policy network to make better actions. 
We will also extend EAR to consider explore--exploit balance which is the key problem for traditional interactive recommendation system.
%extend EAR with utterance understanding and response generation to explore its robustness in handling language understanding errors. 
Lastly, we will deploy our system to online applications that interact with real users to gain more insights for further improvements. 
%In order to model user feedback more effectively, a fundamental problem is to have a more realistic dataset and interactive environment for conversational recommendation.

\textbf{Acknowledgement}:
This research is part of NExT++ research and also supported by the National Natural Science Foundation of China (61972372).
NExT++ is supported by the National Research Foundation, Prime Minister's Office, Singapore under its IRC@SG Funding Initiative.
We would like to thank the anonymous reviewers for their valuable reviews. 

\vspace{-10pt}
%which is hacord to be accessed by experiment results.

%In order to model user feedback more effectively, a fundamental problem is to have a more realistic dataset and interactive environment for conversational recommendation.


%which is hacord to be accessed by experiment results.


==> ear-arxiv-new/Exp.tex <==
\section{Experiments}
EAR \footnote{Datasets, source code and demos at our project homepage: https://ear-conv-rec.github.io} is built based on the guiding ideology of interaction between the CC and RC. To validate this ideology, we first evaluate the whole system to examine the overall effect brought by the interaction. Then, we perform ablation study to investigate the effect of interaction on each individual component. Specifically, we have the following research questions (RQ) to guide experiments on two datasets.
%To have a more clear idea of the effect on each individual component, we isolate each component out to investigate the effect of interaction of each component. Specifically, we have the following research questions (RQ) to guide our exploration.
%extensive interactions between CC and RC. We hypothesize it is such interaction that make the overall effect. In this section, we empirically validate our EAR model on two datasets. First, we investigate its eventual effect of the interaction performance. Second, we examine the effect of the interaction on each component by performing ablation study for each component.
%To validate our EAR method, we propose the subsequent research questions to guide our empirical studies.
\begin{itemize}[leftmargin=*]
	\item \textbf{RQ1.} How is the overall performance of EAR comparing with existing conversational recommendation methods?
	\item \textbf{RQ2.} How do the attribute-aware BPR and multi-task training of the \textit{estimation} stage contribute to the RC?
	\item \textbf{RQ3.} Is the state vector designed for the CC in the \textit{action} stage appropriate?	
	\item \textbf{RQ4.} Is the online model update of the \textit{reflection} stage useful in obtaining better recommendation?
\end{itemize}
%In what follows, we first present the experimental settings, followed by the method comparison and the ablation studies to justify the rationality and usefulness of each stage.

%\vspace{-10pt}
\subsection{Settings}
\subsubsection{Datasets}
%Conversational recommendation is a new research area that severely lacks benchmark datasets, therefore we endeavour to propose a pipeline that adapt classic recommendation datasets into multi-round conversational senario. Datasets will be released upon acceptance.
We conduct experiments on two datasets: Yelp\footnote{https://www.yelp.com/dataset/} for business recommendation and LastFM\footnote{https://grouplens.org/datasets/hetrec-2011/} for music artist recommendation.
%another dataset is Last.FM Dataset  which is usually used for online recommendation~\cite{wu2016contextual,wu2018learning}.
%The Yelp dataset contains information for restaurant in different cities. The LastFM Dataset is for artist recommendation.
First, we follow the common setting of recommendation evaluation~\cite{NCF,BPR} that reduces the data sparsity by pruning the users that have less than 10 reviews. We split the user--item interactions in the ratio of 7:2:1 for training, validation and testing.
Table~\ref{tab:data} summarizes the statistics of the datasets.
\begin{table}[t]
\caption{Dataset statistics.}
\vspace{-5pt}
\begin{tabular}{|l|l|l|l|l|}
\hline\small
\textbf{Dataset} & \#\textbf{users} & \#\textbf{items} & \#\textbf{interactions} & \#\textbf{attributes}  \\ \hline
Yelp & 27,675      & 70,311  & 1,368,606 & 590     \\ \hline
LastFM            & 1,801      &  7,432 & 76,693 & 33     \\ \hline
\end{tabular}
%\vspace{-5pt}
\label{tab:data}
\vspace{-5pt}
\end{table}


For the item attributes, we preprocess the original attributes of the datasets by merging synonyms and eliminating low frequency attributes, resulting in 590 attributes in Yelp and 33 attributes in LastFM. In real applications, asking about attributes in a large attribute space (e.g., on Yelp dataset) causes overly lengthy conversation. We therefore consider both the binary question setting (on LastFM) and enumerated question (on Yelp). To enable the enumerated question setting, we build a two-level taxonomy on the attributes of the Yelp data. For example, the \textit{parent attribute} of  \{``wine", ``beer", ``whiskey''\} is ``alcohol''. We create 29 such parent attributes on the top of the 590 attributes, such as ``nightlife'', ``event planning \& services'', ``dessert types'' etc. In the enumerated question setting, the system choose one parent attribute to ask. This is to say, we change the size of the output space of the policy network to be $29+1=30$. At the same time, it also displays all its child attributes and ask the user to choose from them (the user can reply with multiple child attributes).
Note that choosing what kinds of questions to ask is an engineering design choice by participants, here we evaluate our model on both settings. %and it is also possible to mix single-choice with multi-choice questions.
%Here we ask binary questions in LastFM and multi-choice questions in Yelp to test EAR in handling both types of questions.
%As discussed in Section~\ref{}, the basic form of our question is to ask whether a user likes an attribute or not. However, in cases where more than hundreds of attributes exist, it is better to ask multiple attribute choice question. Therefore, we manually construct 27 categories for all attributes according to their nature. For example, we construct a category called ``alcohol" where all attributes like falls  ``wine", ``beer" in it.
%In the multi-attributes choice setting, if a model decide to ask an attribute, it asks about the category and lists all element attributes for the user to choose.

\subsubsection{User Simulator For Multi-round Scenario.}
\label{sec:simu}
Because the conversational recommendation is a dynamic process, we follow  ~\cite{zhang2018towards,Sun:2018:CRS:3209978.3210002}) to create a user simulator to enable the CRS training and evaluation.
%mimic the user to simulator conversation history to train user offline recommender model, optimize and evaluate the whole CRS.
%simulate the conversational histories %(note that most existing research on conversational recommendation also simulates conversations~\cite{zhang2018towards,Sun:2018:CRS:3209978.3210002}).
We simulate a conversation session for each observed interaction between users and items. Specifically, given an observed user--item interaction $(u,v)$, we treat the $v$ as the ground truth item to seek for and its attributes $\mathcal{P}_v$ as the oracle set of attributes preferred by the user in this session. At the beginning, we randomly choose an attribute from the oracle set as the user's initialization to the session. Then the session goes in the loop of the ``model acts -- simulator response" process as introduced in Section~\ref{sec:pre}.
% Yisong: add here.
We set the max turn $T$ of a session to 15 and standardize the recommendation list length $\mathcal{V}^{t}$ as 10.

\subsubsection{Training Details}
Following CRM~\cite{Sun:2018:CRS:3209978.3210002},
the training process is divided into offline and online stages. The offline training is to build the RC (i.e., FM) and initialize the policy network (PN) by letting them optimize performance with the offline dialogue history. Due to the scarcity of the conversational recommendation dialogue history, we follow CRM~\cite{Sun:2018:CRS:3209978.3210002} to simulate dialogue history by building a rule-based CRS to interact with the simulator introduced in Section~\ref{sec:simu}. Specifically, the strategy for determining which attribute to ask about is to choose the
% Min: shouldn't it be attribute?
% Wenqiang: Yes. Session closed.
% item
attribute
with the maximum entropy. Each turn, the system chooses the recommendation action with probability $10 / max({|\mathcal{V}|, 10})$ where $\mathcal{V}$ is the current candidate set. The intuition is that the confidence of recommendation grows when the candidate size is smaller. We train the RC to give the ground-truth item and oracle attributes higher ranks given the attribute confirmed by users in dialogue histories, while training the policy to mimic the rule-based strategy on the history. Afterwards, we conduct online training, optimizing the PN by letting EAR interact with the user simulator through reinforcement learning.

We tuned all hyper-parameters on the validation set, and empirically set them as followed:
The embedding size of FM is set as 64.
%, same number for other baseline if it is an embedding-based model.
We employ the multi-task training mechanism to optimize FM as described in Section~\ref{ss:multi-task}, using SGD with a regularization strength of 0.001. The learning rate for the first task (item prediction) and second task (attribute prediction) is set to 0.01 and 0.001, respectively.
%The hidden size we set for the FM model is 64. We first pre-train the FM model with SGD optimizer by learning rate of 0.01, with 0.001 L2 regularization, when the training converges(the AUC of item prediction doesn't increase), we use multi-task learning method to jointly optimize target 1 and target 2. We optimize both target with SGD optimizer, the first one with same learning rate of 0.01, and the second one with learning rate of 0.001.
The size of the two hidden layers in the PN is set as 64.
%We first pre-train the PN as a classifier to give it a warmer start, for which the input is the state vector and the output is the ground truth action.
When the pre-trained model is initialized, we use the REINFORCE algorithm to train the PN.
The four rewards are set as: $r_{suc}$=1, $r_{ask}$=0.1, $r_{quit}$=-0.3, and $r_{prev}$=-0.1, and the learning rate $\alpha$ is set as $0.001$. The discount factor $\gamma$ is set to be 0.7.

%--------
%Wenqiang: integrate below information in training details.
%Yisong: doing.
% Before training the policy network with reinforcement, it is a good strategy to pretrain the policy network with supervised learning in dialogue policy [...]. We also follow [] to simulate dialogue history to pre-train policy network. The history  is simulated by letting a rule-based policy network to interact with the user simulator: it asks the attribute that has the maximum entropy among the candidate items, and the simulator judges whether the asked attribute is within the oracle set.
% %When the number of candidates is between 50 and 100, the simulator chooses to recommend items with a probability of 0.5; when the number is smaller than 50, the simulator will always choose to make a recommendation.
% %The recommendation list size is 10.
% If the recommendation hits the ground truth item $v$, the session is finished, otherwise the process continues.
% %We set the maximum conversation turn to be 15, i.e., $T=15$. %after which the session terminates even the simulator has not hit the ground truth item $v$.
% The system choose to recommend items with a probability inversely proportional to size of candidate item list $\mathcal{V}$, specifically $10 / |\mathcal{V}|$, since a smart strategy is to recommend items when the candidates are small, and be certain to recommend when candidates is less than 10. The simulated conversation data will also be released upon acceptance to facilitate reproduction.

%-------------
%the max-entropy generate 70000 (state, action) pairs to pre-train the policy network as a classifier.

\subsubsection{Baselines.}
As our multi-round conversational recommendation scenario is new, there are few suitable baselines.  We compare our overall performance with the following three:
\begin{itemize}[leftmargin=1mm]
    \item \textbf{Max Entropy}. This method follows the rule we used to generate the conversation history in Section~\ref{sec:simu}. Each turn it asks the attribute that has the maximum entropy among the candidate items. It is claimed in~\cite{dhingra2017towards} that maximum entropy is the best strategy when language understanding is precise. It's worth noting that, in enumerated question setting, the entropy of an attribute is calculated as the sum of its child attributes in the taxonomy (similar approach for attribute preference calculation).
    % , and the attribute preference is calculated in a similar way.
    %Yisong: The claim was strong, so beneficial for us.
    %Yisong: will they attack us for the naive probability of 10/V? If so, we better omit that?
    \item \textbf{Abs Greedy}~\cite{christakopoulou2016towards}. This method recommends items in every turn without asking any question. Once the recommendation is rejected, it updates the model by treating the rejected items as negative examples. According to~\cite{christakopoulou2016towards}, this method achieves equivalent or better performance than popular bandit algorithms like Upper Confidence Bounds~\cite{auer2002using} and Thompson Sampling~\cite{chapelle2011empirical}.% We compare with this model to demonstrate the efficacy of asking attributes in the conversational recommendation scenario.
    \item \textbf{CRM}~\cite{Sun:2018:CRS:3209978.3210002}. This is a state-of-the-art CRS. Similar to EAR, it integrates a CC and RC by feeding the belief tracker results to FM for item prediction, without considering much interactions between them. It is originally designed for single-round recommendation. To achieve a fair comparison, we adapt it to the multi-round setting by following the same offline and online training of EAR.
    %Wenqiang: adding two more baselines if space allows: EAR minus strong FM; EAR minus strong CC.
    %However, it only does single-round recommendation and lacks strategies to account for the rejected recommendation signal.
    %By comparing with this, we aim to prob the efficacy of the deep interaction strategy between CC and RC.
\end{itemize}
%For a fair comparison on the conversational strategy, we employ our FM (multi-task trained) as the recommender model of all methods.
It is worth noting that although there are other recent conversational recommendation methods~\cite{zhang2018towards,nips18/DeepConv,christakopoulou2016towards,Liao:2018}, they are ill-suited for comparison due to their different task settings. For example, \cite{zhang2018towards} focuses on document representation which is unnecessary in our case. It also lacks the conversation policy component to decide when to make what action.  \cite{nips18/DeepConv} focuses more on language understanding and generation. We summarize the settings of these methods in Table~\ref{tab:CRS} and discuss differences in Section~\ref{sec:related}.
%Wenqiang: add comments on new dataset.
%\vspace{-5pt}
% Can't be shorter in this part.
\subsubsection{Evaluation Metrics}
We use the success rate (SR@t)~\cite{Sun:2018:CRS:3209978.3210002} to measure the ratio of successful conversations, i.e., recommend the ground truth item by turn $t$. % Each time of recommendation, the method returns top-10 items.
We also report the average turns (AT) needed to end the session. Larger SR denotes better recommendation and smaller AT denotes more efficient conversation. When studying RC model of offline training, we use the AUC score which is a surrogate of the BPR objective~\cite{BPR}. We conduct one-sample paired t-test to judge statistical significance.% where necessary.

%We use Success Ratio(SR) to evaluate how successful can our CRS to recommend user with his target item. More specifically, SR@K means the cumulative hit ratio at $k-th$ turn.
%We also study the average turn of conversation.

%Although there existing several pieces of conversational recommendation models, most of them are incomparable because they follow different settings.
%~\citet{zhang2018towards} is for conversational search where the main focus is matching the document between queries; ~\cite{nips18/DeepConv} focus on building language understanding and generation; \citet{NCF} focus on multi-model retrieval. Therefore, we does not compare our models with theirs. Instead, we choosing the following model as our baselines.

%\noindent  This is a rule-based method which is used to initialize the the policy network (\emph{c.f.} Sec.~\ref{sec:simu}). %The model keeps asking the attributes that have the max entropy in the  candidate. When the number of candidate is between 50 and 100, the CRS chooses to recommend items with the probability of 0.5; when the number of candidate is smaller than 50, model will always choose to make a recommendation.\\
%The entropy for an attribute i with m value is calculated as:
%\begin{equation}
%Entropy(P_{i}) = \sum_{1}^{m} - Prob({P}_{i}_{j}) \cdot log(Prob({P}_{i}_{j}))
%\end{equation}
%\noindent \textbf{Naive Greedy.} It keep recommending top items at any time with update.\\
%\textbf{Abs Greedy.}~\cite{christakopoulou2016towards}.

%\textbf{LinUCB} Proposed by~\cite{}. This is a standard online learning algorithm which balances explore-exploit problem.\\



%\subsection{Evaluation Metrics}
%\subsubsection{Offline Estimator Evaluation}
%We use AUC(Area Under Curve) to evaluate the performance of the offline trained estimator. More specifically, given a user and his partially known preference $P_{K}$, we use AUC to evaluate where does the estimator rank the target item in the $CanList$ and where it rank the ground truth unknown feature $P_{U}$ given $P_{K}$.
%\subsubsection{Interactive Action Evaluation}
%%%%%%Wenqiang: detail the evaluation metrics.
%%%%%TODO

\subsection{Performance Comparison~(RQ1)}

\vspace{-15pt}

\begin{figure}[htbp]
\begin{minipage}[t]{0.47\linewidth}
    \includegraphics[width=\linewidth]{Yelp-comp.png}
    %\caption{caption1}
    \label{f1}
\end{minipage}%
    \hfill%
%\hspace{+0.1pt}
    %\hspace{+0.1pt}
\begin{minipage}[t]{0.47\linewidth}
    \includegraphics[width=\linewidth]{lastfm-comp.png}
    %\caption{caption2}
    \label{f2}
\end{minipage}
\vspace{-15pt}
\caption{Success Rate* of compared methods at different conversation turns on Yelp and LastFM (RQ1).}
\label{fig:overall}
\vspace{-5pt}
\end{figure}

\begin{table}[t]
\caption{SR@15 and AT of compared methods. $^*$ denotes that improvement of EAR over other methods is statistically significant for $p<0.01$ (RQ1).}
\vspace{-5pt}
\label{tab:result}\small
\begin{tabular}{m{2.2cm}|m{1cm}|m{0.8cm}|m{1cm}|m{0.8cm}}\hline
& \multicolumn{2}{c|}{\textbf{LastFM}}  & \multicolumn{2}{c}{\textbf{Yelp}}\\ \hline
 & \textbf{SR@15}    & \textbf{AT} & \textbf{SR@15}    & \textbf{AT} \\ \hline
Abs Greedy &0.209 &13.63 & 0.271 & 12.26  \\ \hline
Max Entropy & 0.290 &13.61 &0.919 &5.77 \\ \hline
CRM & 0.325 & 13.43 & 0.923 & 5.33 \\ \hline
\textbf{EAR}  & \textbf{0.429}* & \textbf{12.45}* & \textbf{0.971}* & \textbf{4.71}*\\ \hline
\end{tabular}
\label{tab:main}
\vspace{-10pt}
\end{table}

Figure~\ref{fig:overall} shows the recommendation Success Rate* (SR*) @t at different turns ($t=1$ to 15), SR* denotes the comparison of each method against the strongest baseline CRM,
% Min BUG: shouldn't it be y=0?
% which serves as the x=0
% Wenqiang: session closed.
indicated as $y=0$
in the figure. Table~\ref{tab:main} shows the scores of the final success rate and the average turns. As can be clearly seen, our EAR model significantly outperforms other methods. This validates our hypothesis that considering extensive interactions between the CC and RC is an effective strategy to build conversational a recommender system. We also make the following observations:

Comparing with Abs Greedy, the three attribute-based methods (EAR, Max Entropy and CRM) have nearly zero success rate at the beginning of a conversation ($t<2$). This is because these methods tend to ask questions at the very beginning. %which is proven to be a useful strategy.
As the conversation goes, Abs Greedy (which only recommends items) gradually falls behind the attribute-based methods, demonstrating the efficacy of asking attributes in the conversational recommendation scenario.
%Regarding Abs Greedy method, we On Yelp, Abs Greedy achieves a much weaker performance than the other three attribute-based methods (note that Abs Greedy only recommends items). In contrast, its performance on LastFM is much better and is comparable with other methods.
Note that Abs Greedy has much weaker performance on Yelp compared to LastFM. The key reason is the setting of Yelp is to ask enumerated question, and user's response with multiple finer-grained attributes sharply shrinks the candidate items.
%which have much fine-grained attributes as answers. These fine-grained attributes can effective prone less qualified candidates and largely improve the performance.

CRM generally underperforms our EAR methods. One of the key reasons is that its state vector cannot help CC to learn sophisticated strategy to ask and recommend, especially in a much larger action space, i.e., the number of attributes (nearly 30 in our experiments versus 5 in theirs~\cite{Sun:2018:CRS:3209978.3210002}). This result suggests that in a more complex  \textit{multi-round} scenario where the CC needs to make a comprehensive utilization of both the CC (e.g., considering dialogue histories) and RC (considering statistics like attribute preference estimation) when formulating a recommendation strategy. %, highlighting the importance of the interaction between CC and RC.

Interestingly, % we found in
Figure~\ref{fig:overall} indicates that in Yelp, EAR's gain over CRM enlarges in Turns~1--3, shrinks in Turns~4--6 and widens again afterwards. However, in LastFM it has a steadily increasing gain. This interesting phenomenon reveals that our EAR system can learn different strategies in different settings. In the Yelp dataset, the CRS asks enumerated questions where the user can choose finer-grained attributes, resulting a sharp reduction in the candidate space. The strategy that the EAR system learns is more aggressive: it attempts to ask attributes that can sharply shrink the candidate space and make decisive recommendation at the beginning turns when it feels confident. If this aggressive strategy fails, it changes to a more patient strategy to ask more questions without recommendations, causing less success in the medial turns (e.g., Turns~5--7). However, this strategy pays off in the long term, making recommendation more successful in the latter half of conversations (e.g., after Turn~7). At the same time, CRM is only able to follow the strategy of trying to ask more attributes at the beginning and making recommendations later. In the LastFM dataset, the setting is limited to binary attributes, leading to less efficiency in reducing candidate space. Both EAR and CRM adapt and ask more questions at the outset before making recommendations. However, as EAR incorporates better CC and RC to model better interaction, it significantly outperforms CRM.

%vspace{-5pt}

%Enumerated question (i.e. Yelp's setting) can receive user's feedback with multiple finer grained attributes, resulting a sharply reduced candidate space. Accordingly, EAR can be decisive to recommend when the candidate has a sharp shrinking (as Turn 3 in Yelp), and is patient to ask more question in cases like previous recommendation was rejected to achieve optimum long term reward.

%length is small enough (as Turn 3 in Yelp), and is patient to ask more question in cases like previous recommendation was rejected to achieve optimum long term reward, demonstrating the effectiveness of combining CC and RC's information for decision making in multi-turn scenario in two question settings.

% This interesting phenomenon is an evidence that EAR integrated smarter strategy in two typical \textit{multi-round} interaction circumstances.
% %the Let us walk through the SR curve of EAR and CRM in Yelp in Figure~\ref{fig:overall},
% First, when candidate items shrinks sharply as user may enumerate multiple desired attributes, EAR is decisive to recommend items when it has high confidence. This results to significant improvement in SR@2-3.
% %Figure~\ref{fig:cs-1} represents a circumstance where candidate items shrinks sharply because user answers enumerative question, and EAR is able to take decisive action to recommend items when it has high confidence which results to significant improvement in SR@2-3.
% In contrast, when candidate items doesn't shrink sharply or previous recommendation is not accepted, EAR is patient to ask more question which results to shrunken gain in SR@4-6. Nevertheless, such combination of decisiveness and patience helps EAR achieves the best overall result as improvement enlarges in SR@7-15, validating that EAR is better at handling \textit{multi-round} recommendation scenario.

%Yisong: case study?

% \begin{figure}[t]
%     \centering
%     \subfigure{
% 	\includegraphics[width=0.5\textwidth]{cs-1.pdf}}\vspace{-5pt}
%     \caption{EAR is decisive to recommend when it has high confidence}\label{fig:cs-1} \vspace{-5pt}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure{
% 	\includegraphics[width=0.5\textwidth]{cs-2.pdf}}\vspace{-5pt}
%     \caption{EAR is patient to ask more questions to adjust estimation}\label{fig:cs-2} \vspace{-5pt}
% \end{figure}


\subsection{Effectiveness of Estimation Designs (RQ2)}
\label{sec:main_result}
There are two key designs in the \text{estimation} stage that trains the recommendation model FM offline: the attribute-aware BPR that samples negatives with attribute matching considered, and the multi-task training that jointly optimizes item prediction and attribute prediction tasks. Table \ref{tab:RS_offline} shows offline AUC scores on the two tasks of three methods: FM, FM with attribute-aware BPR (FM+A), and FM+A with multi-task training (FM+A+MT).

\begin{table}[t]
\label{tab:RS_offline}
\small
\caption{Offline AUC score of FM, FM with attribute-aware BPR (FM+A) and with multi-task training for item recommendation and attribute prediction (FM+A+MT). $^*$ denotes that improvement of FM+A+MT over FM and FM+A is statistically significant for $p<0.01$ (RQ2).}
\vspace{-5pt}
\begin{tabular}{m{1.3cm}|>{\centering\arraybackslash}m{1.3cm}|>{\centering\arraybackslash}m{1.3cm}|>{\centering\arraybackslash}m{1.3cm}|>{\centering\arraybackslash}m{1.3cm}}\hline
& \multicolumn{2}{c|}{\textbf{LastFM}}  & \multicolumn{2}{c}{\textbf{Yelp}}\\ \hline
 & \textbf{Item}   & \textbf{Attribute}  & \textbf{Item}  & \textbf{Attribute}  \\ \hline
FM & 0.521 & 0.727 & 0.834 & 0.654\\ \hline
FM+A & 0.724 & 0.629 & 0.866 & 0.638\\ \hline
FM+A+MT & \textbf{0.742}* & \textbf{0.760}* & \textbf{0.870}* & \textbf{0.896}* \\ \hline
\end{tabular}
\vspace{-8pt}
\label{tab:RS_offline}
\end{table}

%This section examines the offline performance of  recommendation component in the \emph{estimation} stage, providing evidences on how our model address the challenges in the conversation scenario. Table~\ref{tab:RS_offline} demonstrates the AUC of item and attribute prediction.
As can be seen, the attribute-aware BPR significantly boosts the performance of item ranking, being highly beneficial to rank the ground truth item high. Interestingly, it harms the performance of attribute prediction, e.g. on lastFM, FM+A has a much lower AUC score (0.629) than FM (0.727).
The reason might be that the attribute-aware BPR loss guides the model to specifically fit to item ranking in the candidate list. Without an even optimization enforced for the attribute prediction task, it may suffer from poor performance. This implies the necessity of explicitly optimizing the attribute prediction task.
%., digressing from capture general similarity between attributes.
As expected, the best performance is achieved when we add multi-task training on. FM+A+MT significantly enhances the performance of both tasks, validating the effectiveness and rationality of our multi-task training design.
%However, when multi-task training is adopted, both the item and attribute prediction becomes better.
% \vspace{-5pt}

\subsection{Ablation Studies on State Vector (RQ3)}

% yisong: in this section, we can talk about more, how RC helps CC?

%The dialogue action is one of the key task for a CRS. The experiment result in Section~\ref{sec:main_result}

%As discussed in performance comparison in Section~\ref{sec:main_result}, the worse performance of CRM than Max Entropy validates our hypothesis that the belief tracker result is not sufficient for decision making in conversational recommendation.
What information helps in decision making? Let us examine the effects of the the four forms of information included in EAR state vector $\textbf{s}$ (Equation~\ref{eq:state}), by ablating each information type from the feature vector (Table~\ref{ablation}).

% \begin{table}[t]
%     \small
%     \centering
%     \begin{threeparttable}
%     %\caption{Performance of removing one component of the state vector (Equation~\ref{eq:state}) from our EAR. $\textbf{s}_{ent}$, $\textbf{s}_{pre}$, $\textbf{s}_{his}$ and $\textbf{s}_{len}$ denote the state vector that encodes the attribute entropy, user attribute preference, conversation history, and candidate list length, respectively.}\vspace{-8pt}\label{tab:sta_vec_abla}
%     \caption{Performance of removing one component of the state vector (Equation~\ref{eq:state}) from our EAR. (RQ 3)}
%     \setlength{\abovecaptionskip}{0.15cm}
%     \label{results of relation ablation}
%     \begin{tabular}{lccc|c}
%     \toprule\small
%     \multirow{}{}{}&
%     \multicolumn{3}{c}{\textbf{Yelp}}&\cr
%     \cmidrule(lr){2-5}
%     &\textbf{SR@5}&\textbf{SR@10}&\textbf{SR@15}&\textbf{AT}\cr
%     \midrule
%     \textbf{EAR} w/o \textbf{s}_{ent}$ &0.614&0.895&0.969&4.81\cr
%     \textbf{EAR} w/o \textbf{s}_{pre}$ &0.596&0.857&0.959&5.06\cr
%     \textbf{EAR} w/o \textbf{s}_{his}$ &0.624&0.894&0.949&4.79\cr
%     \textbf{EAR} w/o \textbf{s}_{len}$ &0.550&0.846&0.952&5.44\\ \hline
%     \textbf{EAR} &\bf0.629&\bf0.907&\bf0.971&\bf4.71\cr
%     \midrule
%     \multirow{}{}{}&
%     \multicolumn{3}{c}{\textbf{LastFM}}&\cr
%     \cmidrule(lr){2-5}
%     &\textbf{SR@5}&\textbf{SR@10}&\textbf{SR@15}&\textbf{AT}\cr
%     \midrule
%     \textbf{EAR} w/o \textbf{s}_{ent}$ &\bf 0.051&0.190&0.346&12.82\cr
%     \textbf{EAR} w/o \textbf{s}_{pre}$ &0.024&0.231&0.407&12.55\cr
%     \textbf{EAR} w/o \textbf{s}_{his}$ &0.021&0.236&0.424&12.50\cr
%     \textbf{EAR} w/o \textbf{s}_{len}$ &0.013&0.230&0.416&12.56\\ \hline
%     \textbf{EAR} & 0.020&\bf 0.243&\bf0.429&\bf12.45\cr
%     \bottomrule
%     \end{tabular}\vspace{-10pt}
%     \end{threeparttable}
% \end{table}

\begin{table}[t]
\small
\label{results of relation ablation}\small
\caption{Performance of removing one component of the state vector (Equation~\ref{eq:state}) from our EAR. $^*$ denotes that improvement of EAR over model with removed component is statistically significant for $p<0.01$ (RQ 3).}
\vspace{-5pt}
\begin{tabular}{m{0.7cm}|>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}
|>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}}\hline
& \multicolumn{4}{c|}{\textbf{Yelp}}  & \multicolumn{4}{c}{\textbf{LastFM}}\\ \hline
 & SR@5   & SR@10  & SR@15  & AT & SR@5   & SR@10 & SR@15  & AT\\ \hline
$-\textbf{s}_{ent}$ &0.614&0.895&0.969&4.81 &\bf 0.051&0.190&0.346&12.82 \\ \hline
$-\textbf{s}_{pre}$ &0.596&0.857&0.959&5.06&0.024&0.231&0.407&12.55\\ \hline
$-\textbf{s}_{his}$ &0.624&0.894&0.949&4.79&0.021&0.236&0.424&12.50 \\ \hline
$-\textbf{s}_{len}$ &0.550&0.846&0.952&5.44&0.013&0.230&0.416&12.56 \\ \hline
\textbf{EAR} &\bf0.629*&\bf0.907*&\bf0.971*&\bf4.71* & 0.020&\bf 0.243*&\bf0.429*&\bf12.45*\\ \hline
\end{tabular}
\label{ablation}
\vspace{-10pt}
\end{table}


Comparing the performance drop of each method, we uncover differences that corroborate the intrinsic difference between the two conversational settings. The most important factor is question type: i.e., $\textbf{s}_{ent}$ for LastFM (binary question) and $\textbf{s}_{len}$ for Yelp (enumerated question). The entropy($\textbf{s}_{ent}$) information is crucial for LastFM, it is in line with the claim in ~\cite{dhingra2017towards} that the maximum entropy is the best strategy when language understanding is precise. % and our experiment results shown in Table~\ref{tab:result} and Figure~\ref{fig:overall} that Max Entropy turns out to be a strong baseline.
%because single-value question reduces less candidate items compared to multi-value question, thus requires asking more precise attributes.
If we ablate $\textbf{s}_{ent}$ on LastFM, although it reaches 0.051 in SR@5, future SR greatly suffers, due to the system's over-agressiveness to recommend items before obtaining sufficient relevant attribute evidence.
%The importance of entropy is in line with our experiment results shown in Table~\ref{tab:result} and Figure~\ref{fig:overall} that Max Entropy turns out to be a strong baseline, and also both the CC of CRM and EAR are initialized upon it.
As for the enumerated question setting (Yelp), the candidate list length ($\textbf{s}_{len}$) is most important, because the candidate item list shrinks more sharply and $\textbf{s}_{len}$ is helpful when deciding when to recommend.

%The the attribute entropy information is the most important factor, as removing it sharply degrades the performance in all cases.
%This is in line with our experiment results shown in Table~\ref{tab:result} and Figure~\ref{fig:overall} that Max Entropy turns out to be the strongest baseline.
Apart from entropy and candidate list length, the remaining two factors -- i.e., attribute preference, conversation history -- both contribute positively.
Their impact is sensitive to datasets and metrics. For example, the attribute preference ($\textbf{s}_{pre}$) strongly affect SR@5 and SR@10 on Yelp, but does not show significant impacts for SR@15.
% Min: this sentence says nothing.  Do you need it?
% Wenqiang: This is to give an excuse on our inability of explain the inconsistency of the ablation study.
% Session closed.
This inconsistency provides an evidence for the intrinsic difficulty of decision making in the conversational recommendation scenario, which however has yet to be extensively studied.
% \vspace{-5pt}
\subsection{Investigation on Reflection (RQ4)}


\begin{table}[t]
\small
\caption{Performance after removing the online update module in the reflection stage. $^*$ denotes that improvement of EAR over removing update module is statistically significant for $p<0.01$ (RQ4).}\label{tab:RQ4}
\vspace{-5pt}
\begin{tabular}{m{1cm}|>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}
|>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}>{\arraybackslash}m{0.6cm}}\hline
& \multicolumn{4}{c|}{\textbf{Yelp}}  & \multicolumn{4}{c}{\textbf{LastFM}}\\ \hline
 & SR@5   & SR@10  & SR@15  & AT & SR@5   & SR@10 & SR@15  & AT\\ \hline
-\textbf{update} &0.629& 0.905 & 0.970 & 4.72 &0.020& 0.217 & 0.393 & 12.67 \\ \hline
\textbf{EAR} &\bf0.629&\bf0.907&\bf0.971&\bf4.71 & \bf0.020&\bf 0.243*&\bf0.429*&\bf12.45*\\ \hline
\end{tabular}
\vspace{-10pt}
\end{table}

\begin{figure}[t]
    \centering
%    \subfigure{
%    \includegraphics[width=0.35\textwidth]{update-lastfm-2.pdf}}\hspace{+20pt}
    \subfigure{
    % Min: redo figure to use wider aspect ratio and then fix the includegraphics options accordingly.
	%\includegraphics[width=\columnwidth,height=2.5cm]{update-yelp-3.pdf}}\vspace{-10pt}
	\includegraphics[height=3.6cm]{update-yelp-3.png}}\vspace{-5pt}
    \caption{Percentage of bad updates w.r.t. the offline model's AUC on the users on Yelp (RQ4).
    }\label{fig:update}
    \vspace{-10pt}
\end{figure}


\begin{table*}[t]\centering
\caption{Recent conversational recommender summary: 1) whether it asks about attributes, 2) question space, 3) any explicit strategy w.r.t. recommendation timing, 4) whether it considers multi-round recommendations, and 5) its main focus.}\label{tab:CRS}\vspace{-8pt}
  \small
  \begin{tabular}{m{2.8cm}|>{\centering\arraybackslash}m{0.8cm}|>{\centering\arraybackslash}m{2.4cm}|>{\centering\arraybackslash}m{1.4cm}|>{\centering\arraybackslash}m{2cm}|m{6.5cm}}\hline
                 & \textbf{1. Q?}  & \textbf{2. Question Space} & \textbf{3. Explicit} & \textbf{4. Multi-round} & \textbf{5. Main Focus} \\ \hline
Online bandits~\cite{christakopoulou2016towards,wu2016contextual,wu2018learning}& $\times$ & N.A. & $\times$ & $\checkmark$ &   Exploration-exploitation trade-off in item selection \\ \hline
REDIAL (NIPS'18)~\cite{nips18/DeepConv} &  $\checkmark$ & Free texts & $\times$ &$\checkmark$ & End-to-end generation of natural language response \\ \hline
KMD (MM'18)~\cite{Liao:2018} & $\checkmark$ & Free texts & $\times$ & $\checkmark$ & End-to-end generation of text and image response \\ \hline
Q\&R (KDD'18)~\cite{christakopoulou2018q}        & $\checkmark$  & Attributes & $\times$ &  $\times$  & Question asking and single-round recommendation \\ \hline
MMN (CIKM'18)~\cite{zhang2018towards} &  $\checkmark$  &  Attributes  &  $\times$  & $\checkmark$  & Attribute-product match in conversational search \\ \hline
CRM (SIGIR'18)~\cite{Sun:2018:CRS:3209978.3210002}       & $\checkmark$   & Attributes  &  $\checkmark$    &    $\times$   &  Shallow combination between CC and RC  \\ \hline
VDARIS (KDD'19)~\cite{yu2019visual}       & $\times$   & N.A.  &  $\times$    &    $\checkmark$   &  User's click and comment on recommended items \\ \hline
%ConUCB (arXiv'19)~\cite{zhang2019toward}       & $\checkmark$   & Attributes  &  ?    &    $\checkmark$   &  Ask one attribute or rec one item each turn \\ \hline
%DCR (arXiv'19)~\cite{liao2019deep}       & $\checkmark$   & Attributes  &  ?    &    ?   &  Dialogue generation \\ \hline
EAR (our method) & $\checkmark$ & Attributes &$\checkmark$ &$\checkmark$ & Deep interaction between CC and RC  \\ \hline
\end{tabular}
%\vspace{-15pt}
\vspace{-5pt}
\end{table*}

%This RQ studies the efficacy of our updating strategy in the \emph{reflection} stage.
To understand the impact of online update in the reflection stage, we start from the ablation study.  Table~\ref{tab:RQ4} shows the variant of EAR that removes online update. We find that the trends do not converge on two datasets: the updating strategy helps a lot on LastFM but has very minor effect on the Yelp dataset.
%where the full EAR model is compared with its variant without updating when a list of items get rejected. However, the trends shown in Table~\ref{tab:update_abl} does not converge on two dataset: the updating strategy helps a lot in LastFM dataset but have no effect on the Yelp dataset.

Questioning this interesting phenomenon, we examine the individual items on Yelp.
We find that the updating does not always help ranking, especially when the offline model already ranks the ground truth item high (but not at top 10).
%the ground truth item to get high ranks when using the rejected item to update the model.
%For instances that has a fair high rank but not ranks in top 10, our update operation might even lower their original rank.
In this case, doing updates is highly likely to pull down the ranking position of the ground truth item.
To gain statistical evidence for this observation,
we term such updates as \textit{bad updates}, and show the percentage of bad updates with respect to the offline model's AUC on the users. As seen from Figure~\ref{fig:update}, there is a clear positive correlation between bad updates and AUC score. For example, $\sim$3.5\% of the bad updates come from users with an offline AUC of 0.9.
%we show the percentage of \textit{bad updates} (that pull down the ranking position of the ground truth item)
%we show the AUC distribution of the instances whose ranking is lower by the updating operation.
%This results in Figure~\ref{fig:update} which show the instance with higher AUC is more likely be negatively affected by our updating method.

This explains why online update works well for LastFM, but not for Yelp:
our recommendation model has a better performance on Yelp than LastFM (0.870 v.s. 0.742 in AUC as shown in Table~\ref{tab:RS_offline}).
This means the items on Yelp are more likely to get higher AUC, resulting in worse updates.
% Going beyond drawing such a conclusion,
%However, instead of drawing a conclusion,
More such observations and analyses will help further the community understanding the efficacy of online updates.
%initialization of more discussion on the online updating techniques.
Although bandit algorithms have devoted to exploring this question~\cite{kuleshov2014algorithms,chu2011contextual,li2016collaborative,gentile2014online,wu2016contextual}, the issue has largely been unaddressed in the context of conversational recommender system.


==> ear-arxiv-new/Intro.tex <==

\section{Introduction}
\label{sec:introduction}

% Min: BUG GLOBAL: you all should relate this to "concept learning" and the "Find-S" algorithm in fundamental machine learning (version space, instance space, etc).
% Wenqiang: addressed. After discussing with Min, we find it OK to miss the notion of concept learning and Find-S algorithm.

% With the increase in the amount of published information, 
% ~\cite{MF,rendle2010factorization,BPR,NCF,CDL,ACF,sigir/EbesuSF18}
Recommender systems are emerging as an important means of facilitating users' information seeking~\cite{MF,BPR,NCF,ACF}. However, much of such prior work in the area solely leverages the offline historical data to build the recommender model (henceforth, the {\it static recommender system}). This offline focus causes the recommender to suffer from an inherent limitation in the optimization of offline performance, which may not necessarily match online user behavior. User preference can be diverse and often drift with time; and as such, it is difficult to know the exact intent of a user when he uses a service even when the training data is sufficient. %For example, a YouTube user has watched many videos related to multiple topics such as comedy, science, and movie trailers. When the user starts a session in YouTube, a recommendation system has to recommend all the three types of videos despite what she wants currently, resulting in imprecise or even unsatisfactory recommendations.  

%The aforementioned intrinsic limitations enforces the next generation of recommender systems to be able to dynamically obtain user preference when doing recommendation. Fortunately, the rapid development of dialogue techniques [...] bring an unprecedented opportunity to this revolution, enabling the raise of the {\it conversational recommender system} (CRS). %As an emerging research topic, the problem setting for CRS is still open. 

The rapid development of conversational techniques~\cite{nips18/DeepConv,Liao:2018,sigir18/chatmore,acl18/sequicity,jin2018explicit} brings an unprecedented opportunity that allows a recommender system to dynamically obtain user preferences through conversations with users. This possibility is envisioned as the {\it conversational recommender system} (CRS), for which the community has started to expend effort in exploring its various settings. \cite{zhang2018towards} built a conversational search engine by focusing on document representation. 
\cite{nips18/DeepConv} developed a dialogue system to suggest movies for cold start users, contributing to language understanding and generation for the purpose of recommendation, but does not consider modeling users' interaction histories (e.g., clicks, ratings).
In contrast, \cite{christakopoulou2018q} does considers user click history in recommending, but their CRS only handles single-round recommendation. That is, their model considers a scenario in which the CRS session terminates after making a single recommendation, regardless of whether the recommendation is satisfactory or not. While a significant advance, we feel this scenario is unrealistic in actual deployments.

%We in this paper consider a {\it multi-round attribute-aware} setting: a CRS can choose two types of actions --- either explicitly ask whether a user likes a certain attribute of items (denoted as {\it ask}) or recommend a list of items (denoted as {\it recommend}) --- for each dialogue turn. The goal is to hit the user desired item within less turns as the user has only limited patience ({\it c.f.} Sec~\ref{sec:pre} for details). Note that, the {\it multi-round} emphasize that a CRS is allowed to take further actions even its recommendation is rejected. This setting is more realistic and challenging than existing works~\cite{zhang2018towards,christakopoulou2018q,Sun:2018:CRS:3209978.3210002} where a CRS makes a recommendation once after which a dialogue session should be terminated regardless whether users accept the recommendation.
In particular, we believe CRS models should inherently adopt a {\it multi-round} setting: a CRS converses with a user to recommend items based on his click history (if any). At each round, the CRS is allowed to choose two types of actions --- either explicitly asking whether a user likes a certain item attribute or recommending a list of items. In a session, the CRS may alternate between these actions multiple times, with the goal of finding desirable items while minimizing the number of interactions.
%({\it c.f.} Sec~\ref{sec:pre} for details)
This multi-round setting is more challenging than the single-round setting, as the CRS needs to strategically plan its actions. The key in performing such planning, from our perspective, lies in the interaction between the conversational component (CC; responsible for interacting with the user) and the recommender component (RC; responsible for estimating user preference -- e.g., generating the recommendation list). We summarize three fundamental problems toward the deep interaction between CC and RC as follows:
\begin{itemize}[leftmargin=1mm]
    \item \textit{What attributes to ask?} 
    A CRS needs to choose which attribute to ask the user about. For example, in music recommendation, it may ask ``Would you like to listen to classical music?'', expecting a binary yes/no response\footnote{Note that it is possible to compose questions eliciting an enumerated response; i.e., ``Which music genre would you consider? I have pop, funk ...''. However, this is a design choice depending on the domain requirements. In describing our method, we consider the basic single-attribute case.  However in experiments, we also justify the effectiveness of EAR in asking such enumerated questions on Yelp. For the purpose of exposition, we have chosen to avoid open questions that do not constrain user response for now.  Even interpreting user responses to such questions is considered a challenging task~\cite{chen2018hierarchical}.}. 
    If the answer is ``yes'', it can focus on items containing the attribute, benefiting the RC by reducing uncertainty in item ranking. However, if the answer is ``no'', the CRS expends a conversation turn with less gain to the RC. To achieve the goal of hitting the right items in fewer turns, the CC must consider whether the user will like the asked attribute. This is exactly the job of the RC which scrutinizes the user's historical behavior. %Moreover, an effective question should help the RS reduce the uncertainty in ranking items. Thus, asking good questions requires the interaction between CS and RS.

    \item \textit{When to recommend items?} % After several question turns, 
% Min: generated by "RS"?  Is it supposed to be "RC"?
    With sufficient certainty, the CC should push the recommendations generated by the RC. 
    A good timing to push recommendations should be when 1) the candidate space is small enough; when 2) asking additional questions is determined to be less useful or helpful, from the perspective of either information gain or user patience; and when 3) the RC is confident that the top recommendations will be accepted by the user. Determining the appropriate  timing should take both the conversation history of the CC and the preference estimation of the RC into account. 
    \item \textit{How to adapt to users' online feedback?} After each turn, the user gives feedback; i.e., ``yes''/``no'' to a queried attribute, or an ``accept''/``reject'' the recommended items. (1) For ``yes'' on the attribute, both user profile and item candidates need to be updated to generate better recommendations; this requires the offline RC training to take such updates into account. (2) For ``no', the CC needs to adjust its strategy accordingly. (3) If the recommended items are rejected, the RC model needs to be updated to incorporate such a negative signal. Although adjustments seem only to impact either the RC or the CC, we show that such actions impact both.  
\end{itemize}

Towards the deep interaction between CC and RC, we propose a new solution named \textit{Estimation--Action--Reflection} (EAR), which consists of three stages. Note that the stages do not necessarily align with each of the above problems. 
%\begin{enumerate}[leftmargin=*]
(a) Estimation, which builds predictive models offline to estimate user preference on items and item attributes. 
%It provides support for the conversational strategy that determines whether to ask/recommend and what questions to ask about item attributes. 
Specifically, we train a factorization machine~\cite{rendle2010factorization}~(FM) using user profiles and item attributes as input features. Our Estimation stage builds in two novel advances: 1) the joint optimization of FM on the two tasks of item prediction and attribute prediction, and 2) the adaptive training of conversation data with online user feedback on attributes. 
(b) Action, which learns 
the conversational strategy that determines whether to ask or recommend, and what attribute to ask. We train a policy network with reinforcement learning, optimizing the reward of shorter turns and successful recommendations based on the FM's estimation of user preferred items and attributes, and the dialogue history. 
(c) Reflection, which adapts the CRS with user's online feedback. Specifically, when a user rejects the recommended items, we construct new training triplets by treating the items as negative instances and update the FM in an online manner.  
In summary, the main contributions of this work are as follows:
\begin{itemize}[leftmargin=*]
    \item We comprehensively consider a multi-round CRS scenario that is more realistic than previous work, highlighting the importance of researching into the interactions between the RC and CC to build an effective CRS. 
    \item We propose a three-stage solution, EAR, integrating and revising several RC and CC techniques to construct a solution that works well for the conversational recommendation. 
    \item We build two CRS datasets by simulating user conversations to make the task suitable for offline academic research. We show our method outperforms several state-of-the-art CRS methods and provide insight on the task. 
    % Datasets and source code will be released to promote further studies.
\end{itemize}

\vspace{-1mm}

==> ear-arxiv-new/Intro_BAK.tex <==

%% Min: to edit and re-write the intro
With recommendation systems and dialogue agents becoming standard fixtures in workflows, there is an unprecedented opportunity to define how these two technologies can be interwoven.  We envision this intersection as the rise of the {\it conversational recommendation system} (CRS), a system role that allows a dialog agent to recommend items to a user with a naturalistic, dialogic setting, sensitive to the particular mannerisms of human dialog.  We define a basic framework for this scenario, analogous to an exploration–exploitation tradeoff, that allows the system perform two actions: 1) to pose questions (explore) to obtain preferences from the user as well as 2) recommend items (exploit) to the user.

Recommendation systems traditionally use a static user profile, inferred from a user's historical actions, to recommend items for consumption.  While of great success, this approach's key weakness is that it computes an implicit model of the user's need.  What if the agent can interrogate the user directly?  With the advent of dialogue agents, this possibility is more naturally realized through dialog with the user.  

% Could put more emphasis on the difficulty of doing this.
Our CRS framework weaves dialog with recommendation at a fine-grained level, achieving deep interaction.  When the system is uncertain, it queries the user for her preferences to achieve maximal certainty towards relevant recommendations.  When the system reaches sufficient confidence, it recommends items.  This interaction is dynamic, meaning it can switch between both modes in online interactions on a per-turn basis, mimicking human behavior in dialog.  Our proposed {\it Estimation-Action-Reflection} (EAR) asks three key questions in implementing this framework: 1) what questions to ask regarding item attributes, 2) when to recommend items, and 3) how to adapt to the user's feedback.  

We develop our basic EAR framework by describing items as having a set of binary attributes, in which the system can query the user's preference on  selected attribute.  We then further develop the notion of enumerated attributes, where an attribute can take on an enumerated set of values.  Our extended EAR model optimally queries for such enumerated attributes.  We show how a large attribute set can be reduced to a compact set of enumerated attributes to make relevant recommendation efficient.

DONE.


\begin{itemize}
    \item Static has problems
    \item Ask Directly
    \item Semi-formal problem framework.  2 Actions: binary ask or recommend.
    \item Complication: can ask enumerated when attributes are many
\end{itemize}

%% Min: end


%%%Wenqiang initial intro
% Too technical at the very beginning. Too much terminology gives a sharp starting of a paper.
% for example: Min cannot understand what the "induce user preference"
% At the beginning of the introduction, the terminology must be correct. Otherwise, it will confuse the reader.
The rapidly developed conversation systems (CS) bring revolutions to this imprecise and incorrect preference estimation problem. Equipped with CS, a \textbf{conversational recommendation system} (CRS) is able to explicitly ask, verify and even induce users preference through natural languages in an interactive way. For example, in Figure XXX right, a CRS can ask questions like \emph{would you like some electronic devices?} if it is not sure the user's current preferences. This type of interaction is different from multi-armed bandit learning \cite{LinUCB}, an existing interactive recommendation framework which captures user dynamic preference. It keeps recommending items to users and inferring their implicit preferences by observing their actions like clicking, buying and skipping items. However, the preference inferred is also implicit which still suffers from the imprecise and incorrect problem. As a key difference, a CRS does not only infer implicit preferences through user action, but also explicitly consult with them about their preference by asking facets (a.k.a. aspects) of items using natural languages.


We consider a realistic conversational recommendation scenario: a CRS interact with a user by asking features and attempting to recommend items multiple times till he/she chooses satisfying items or leaves the current session. This is more sophisticated
% Wenqiang: sophisticated indicates something incremental.
% wording: fundamentally different.
than existing settings \citet{Sun:2018:CRS:3209978.3210002, zhang2018towards} where a system is designed to make a recommendation at the end of each session. In our scenario, a CRS need a more comprehensive strategy. It may act conservatively, keep asking features until its confidence towards user preference is high enough. Alternatively, it can also take chances to recommend items when achieving a certain level of confidence and adjust its strategy once a recommendation is rejected. The key challenge is to make full use of every single turn to get a satisfactory recommendation within fewer turns because users have limited patience.

As a combination of a RS and a CS, a CRS raises new challenges for both sides. Compared to traditional static recommendation setting, real-time user feedbacks from the CS are available. Such feedbacks indicate user preference explicitly (e.g., telling a facet that he/she prefers) or implicitly (e.g., rejecting a recommendation). How to leverage on both explicit and implicit indications in a CRS still remains to be an open question. On the conversation side, a CRS is also different from traditional task-oriented dialogue systems (cite) which enumeratively check all facets of items with users and demonstrate qualified items to them. A CRS's choice of dialogue action need to consider the estimation of the RS component, with the aim of achieving a successful recommendation within less turns. For example, a CRS does not need to waste a turn to ask a question like \emph{do you like some books?} if the RS thinks he scarcely possible to buy books. Note that we consider a realistic conversational recommendation scenario where a CRS can ask features and recommend items multiple times. This is more sophisticated and challenging than existing settings \citet{Sun:2018:CRS:3209978.3210002, zhang2018towards} where a system is designed to make a recommendation only at the end of each session. This sophisticated scenario  makes the problem even more challenging as a CRS need to make more complicated decisions.

Although some progress has been made along the line of conversational or interactive recommendation, existing research is not focused on the interaction between CS and RS, far from being usable for real-world scenarios. Particularly, state-of-the-art CRS methods either ignore the strategy for when to recommend~\cite{zhang2018towards,nips18/DeepConv} or only consider single-round conversation that recommends items once~\cite{christakopoulou2018q,Sun:2018:CRS:3209978.3210002}. 
To our knowledge, there lacks a unified framework that can jointly solve the three problems well.

Towards the goal of building an effective CRS suitable for practical use, we focus on the extensive interaction between the CS and RS. We propose a new solution named \textit{Estimation-Action-Reflection} (EAR), which consists of three stages: 
%\begin{enumerate}[leftmargin=*]
(a) Estimation, which builds predictive models offline to estimate user preference on items and item attributes. 
%It provides support for the conversational strategy that determines whether to ask/recommend and what questions to ask about item attributes. 
We train a factorization machine~\cite{rendle2010factorization}~(FM) using user profiles and item attributes as input features, with two novelties in: 1) jointly optimizing FM on the two tasks of item prediction and attribute prediction, and 2) revising the training process on conversation data to ensure the model works well with online user feedback on attributes. 
(b) Action, which learns 
the conversational strategy that determines whether to ask or recommend, and what attribute questions to ask. We train a policy network with reinforcement learning, optimizing the reward of short turns and successful recommendations based on FM's estimation of the preferred items, attributes, and dialogue histories. 
(c) Reflection, which adapts the CRS with user online feedback. Specifically, when a user rejects the recommended items, we construct new training triplets by treating the items as negatives and update FM in an online manner.  

%%%%wenqiang initial tro end


%% Wenqiang editted by yisong
\textbf{Static has problems:}
Recommendation systems (RS) have proven to be successful in online services, e.g., suggesting products in e-commerce platforms. Such systems learn users' implicit preferences towards items based on their historical actions (e.g., buying a product). However, the offline static recommender systems have intrinsic limitation. As a usual case, the short of historic data may lead offline learned preference to be imprecise. Even if the historic data is abundant, the learned preference may not conform with user's current need, the estimation for user's preference can be imprecise as the user intention is dynamic and shifting as per recommendation session. An example is illustrated in Figure (XXX left), in a e-commerce platform, a user usually buys four categories of products: electronic devices and clothes. When he visit the platform again, a well-trained RS is supposed to recommend all the two types of products regardless of what the user want to buy at this time, resulting in a imprecise recommendation. In the case where insufficient actions have been recorded for a user, the recommendation will be more imprecise or even incorrect.

\textbf{Ask Directly:}
%Candidate 1
%With the recent improvement of conversational systems including Siri, Cortana, internet users are enjoying the convenience to communicate directly with such systems to accomplish their daily needs or find answer for a question. It is natural to ask, is it possible to conduct the recommendation procedure in an conversational way?
%Candidate 2, Yisong preferred.
In a traditional recommendation scenario, a user can only passively perceive the recommended items from the system and cannot explicitly tell the system her need. In the meantime, the system has difficulty to predict user's current need as user cannot inform it. Therefore there is a gap between the system and user, which can be addressed in a conversational way.

\textbf{Semi-formal problem framework}
To formalize this as a researchable problem, we devise two types of action for the system: raising a question and make recommendation. By raising a question, the user can respond her preference for an attribute to help the system narrow the candidate items. By making recommendation, the user will accept when the desired items is within the recommendation list. We will have a detailed definition in Section 2.


----------------


==> ear-arxiv-new/Method.tex <==
\section{Proposed Methods}
%In order to achieve the successful recommendation within fewer turns, we need to make the full use of each turns to to get feedback from the users.
% Min: don't see any benefit of the first sentence. Omitted.
% Towards the goal of building an effective CRS, we locate the key challenges in the interaction between the RC and CS.
%With the help of the CS, the RC can get real-time explicit feedback about user preference to generate more precise recommendations. Whereas, with the help of RS, the CC can make more wise decision to better solicit user feedback. For example, when choosing which attribute to ask, a good strategy is to avoid asking attributes that a user hardly ever prefers. These intuitions motivate us to develop the three-stage Estimation-Action-Reflection (EAR) solution. In this section, we first give an overview of EAR, following by presenting the techniques of each stage.


%This paper considers a \textit{multi-round} conversational recommendation scenario, where a CRS interacts with the user by asking features and recommending items multiple times until success or the user leaves.
%This is more sophisticated yet realistic than the previous setting~\cite{Sun:2018:CRS:3209978.3210002}, in which the CRS only makes recommendations once and ends the session regardless of success or not.
%Here, we denote one trial of recommendation as a \emph{round}, followed by the work~\cite{christakopoulou2018q}.
%To distinguish our scenario with the settings~\cite{Sun:2018:CRS:3209978.3210002,christakopoulou2018q} that only recommend item once (i.e., single-round), we refer to our scenario as multi-round conversational recommendation. Next we introduce the necessary mathematical notations to describe the scenario that are used cross the paper.

%Let $u\in\mathcal{U}$ denote a user and $v\in\mathcal{V}$ denote an item. Each item has a set of attributes $\mathcal{P}_i$ to describe its properties, such as the music style ``classic'' or ``jazz'' for a song in LastFM, and the tag ``nightlife'', ``'serving burgers'', or ``serving wines'' for a business in Yelp. We denote the set of all attributes as $\mathcal{P}$ and use $p$ to denote a specific attribute.
%Following~\cite{Sun:2018:CRS:3209978.3210002,zhang2018towards}, a CRS session is started with $u$'s specification of a preferred attribute $p^0$.
%After getting the initial preference, the CRS filters out the candidate items that contain the preferred attribute $p^0$.
%Then in each turn $t$ ($t=1, 2, ..., T$ and $T$ denotes the last turn of the session), the CRS needs to choose an action: \textit{recommend} or \textit{ask}:
%\begin{itemize}[leftmargin=*]
%    \item If recommend, we denote the recommended items as $\mathcal{V}^t\subset\mathcal{V}$ and the action as $a_{rec}(\mathcal{V}^t)$. Then the user examines whether the items in $\mathcal{V}^t$ contain his desired item. If the feedback is positive, this session succeeds and can be terminated. Otherwise if the user gives negative feedback, we mark $\mathcal{V}^t$ as \textit{rejected} move to the next turn.
%    \item If ask, we denote the asked attribute as $p^t\in\mathcal{P}$ and the action as $a_{ask}(p^t)$. Then the user gives feedback on whether he prefers items that contain the attribute $p^t$ or not. If the feedback is positive, we add $p^t$ into $\mathcal{P}_u$ to denote the preferred attributes the user in the current session. Otherwise for negative feedback, we mark $p^t$ as \textit{rejected}; regardless of reject or not, we move to the next turn.
%\end{itemize}

% \subsection{EAR Overview}
%As illustrated in Figure~\ref{fig:overview}, o
EAR consists of a recommendation and conversation component (RC and CC) which interact intensively in the three--stage conversational process.
The system starts working at the \emph{estimation} stage where the RC ranks candidate items and item attributes for the user, so as to support the action decision of the CC.
After the \emph{estimation} stage, the system moves to the \emph{action} stage where the CC decides whether to choose an attribute to ask, or make a recommendation according to the ranked candidates and attributes, and the dialogue history.
If the user likes the attribute asked by the RC, the CC feeds this attribute back to the RC to make a new \emph{estimation} again; otherwise, the system stays at the \emph{action} stage: updates the dialogue history and chooses another action. Once a recommendation is rejected by a user, the CC sends the rejected items back to RC, triggering the \emph{reflection} stage where the RC adjusts its estimations.
After that, the system enters the \emph{estimation} stage again.% In the subsequent subsections, we detail each stage.

%In order to gain more evidence quickly to realize the goal that we successfully recommend user's desired item in shortest turns, we summarize three key fundamental problems as discussed in \textbf{Section 1}: 1) What questions to ask regarding item attributes? 2) When to recommend items? 3) How to adapt to user online feedback? we formulate these question mathematically as below, and summarize the key notation in Table 1.

%%%%%%%%%%%%%Wenqiang is working on it%%%%%%%%%%%%%%%
\subsection{Estimation}
% Min: why switch genders of your user?  BUG -- stick to one unless explicitly switching to a new scenario
% Yisong: addressed. As intro uses 'he' and 'his', we use 'his'.
As discussed before, the multi-round conversational scenario brings in new challenges to the traditional RC.
Specifically, the CC interacts with a user $u$ and accumulates evidence on
%his
his
preferred attributes, denoted as  $\mathcal{P}_u=\{p_1,p_2,..,p_n\}$\footnote{We detail how to obtain such data in experiments Section~\ref{sec:simu}.}. % be $u$'s preferred attributes in the conversation session\footnote{We detail how to obtain such data in experiments Section~\ref{sec:simu}.},
%  and now we consider how to train the RC model.
Importantly, different from traditional recommendation methods~\cite{BPR,NCF}, the RC here needs to make full use of $\mathcal{P}_u$ aiming to accurately predict both user's the preferred items and preferred attributes. %achieve two goals:
%\begin{itemize}
%\item Accurately predict the preferred items of $u$.
%\item Accurately predict the preferred item attributes of $u$.
%\end{itemize}
These two goals exert positive influence on EAR, where the first directly contributes to success rate of recommendation, and the second guides the CC to choose better attributes to ask users so as to shorten the conversation.
In the following, we first introduce the basic form of the recommendation method, followed by detail on how we adapt our proposed method to achieve both goals simultaneously.
%and describe how it achieves each goal in our solution.

\subsubsection{Basic Recommendation Method}
we choose the factorization machine (FM)~\cite{rendle2010factorization} as our predictive model due to its success and wide usage in recommendation tasks. However, FM considers all pairwise interactions between input features, which is costly and may introduce undesired interactions that negatively affect our two goals. Thus, we only keep the interactions that are useful to our task and remove the others. Given user $u$, his preferred attributes in the conversation $\mathcal{P}_u$, and the target item $v$, we predict how likely $u$ will like $v$ in the conversation session as:
%We borrow the pair-wise interaction idea from the factorization machine (FM)~\cite{rendle2010factorization} to implement our RS. Letting \textbf{bold} letters, $\mathbf{u}$, $\mathbf{v}$ and $\mathbf{p_i}$ as vector representing the user $u$, item $u$ and the $i-th$ attribute $p_i \in \mathcal{P}$ separately. A FM ranks a item by calculating scores for each item given the user and his/her preferred item:
\begin{equation}
\begin{aligned}
    \hat{y}(u,v,\mathcal{P}_u)= \mathbf{u}^T\mathbf{v}
    %+ \sum_{p_i\in\mathcal{P}_u} \mathbf{u}^T \mathbf{p_i}
    + \sum_{p_i\in\mathcal{P}_u} \mathbf{v}^T \mathbf{p_i},
    %\sum_{i=1}^{n}\sum_{j=i+1}^{n}<\mathbf{p_i},\mathbf{p_j}>
\end{aligned}
%\vspace{-3pt}
\end{equation}
\noindent where $\textbf{u}$ and $\textbf{v}$ denote the embedding for user $u$ and item $v$, respectively, and $\textbf{p}_i$ denotes the embedding for attribute $p_i\in \mathcal{P}_u$. Bias terms are omitted for clarity.
The first term $\mathbf{u}^T\mathbf{v}$ models the general interest of the user on the target item, a common term in FM model~\cite{NCF}.
%The second term $\sum \mathbf{u}^T \mathbf{p_i}$ models user preference on attributes, contributing to the attribute prediction task.
The second term $\sum \mathbf{v}^T \mathbf{p_i}$ models the affinity between the target item and user preferred attributes.
We have also tried to include $v$'s attributes $\mathcal{P}_v$ into FM, but found it brings no benefits. One possible reason is that the item embedding $\textbf{v}$ may have already encoded its attribute information. Thus we also omit it.
%Note that we do not include $v$'s attributes here, since they will introduce noises to the attribute prediction task. The reason is that an interaction between $u$ and $v$ does not mean $u$ prefers all attributes of $v$ --- it is high likely that only partial attributes attract $u$. Thus we only include $\mathcal{P}_u$, the attributes that explicitly reflect $u's$ preference.

To train the FM, we optimize the pairwise Bayesian Personalized Ranking (BPR)~\cite{BPR} objective.
%, which has been shown good performances in item ranking~\cite{ACF}.
%has been shown effective to give higher ranks or the user desired items among $\mathcal{V}$.
Specifically, given a user $u$, it assumes the interacted items (e.g., visited restaurants, listened music) should be assigned higher scores than those not interacted with.
The loss function of traditional BPR is:
\begin{equation}
    L_{bpr} = \sum_{(u,v,v')\in \mathcal{D}_1} -\mbox{ln} \sigma(\hat{y}(u,v,\mathcal{P}_u) - \hat{y}(u,v',\mathcal{P}_u)) + \lambda_{\Theta} \left\|\Theta\right\|^2
\end{equation}
where $\mathcal{D}_1$ is the set of pairwise instances for BPR training, $\mathcal{D}_1 := \{(u, v, v') \mid v' \in \mathcal{V}_{u}^- \}$, where $v$ is the interacted item of the conversation session (i.e., the ground truth item of the session), $\mathcal{V}_{u}^{-}$ := $\mathcal{V} \backslash \mathcal{V}_{u}^{+}$ denotes the set of non-interacted items of user $u$ and $\mathcal{V}_{u}^{+}$ denotes the items interacted by $u$.
$\sigma$ is the sigmoid function, and $\lambda_{\Theta}$ is the regularization parameter to prevent overfitting.

\subsubsection{Attribute-aware BPR for Item Prediction.} However, in our scenario, the emphasis of CRS is to rank the items that contain the user preferred attributes well.
For example, if $u$ specifies ``Mexican restaurant'' as his preferred attribute, a good CRS needs to rank his preferred restaurants among all available Mexican restaurants. %, because other items that do not have the attribute ``Mexican restaurant" should not be considered here.
To capture this, we propose to sample two types of negative examples:
\begin{equation}
%\abovedisplayshortskip
\begin{aligned}
    \mathcal{V}_{u}^{-} := \mathcal{V} \backslash \mathcal{V}_{u}^{+}, \quad
    \widehat{\mathcal{V}}_{u}^- := \mathcal{V}_{cand} \backslash \mathcal{V}_{u}^{+},
\end{aligned}
% \vspace{-5pt}
\end{equation}
where $\mathcal{V}_{u}^{-}$ is the same negative samples as in the traditional BPR setting, i.e., all non-interacted items of $u$.
$\mathcal{V}_{cand}$ denotes the current candidate items satisfying the partially known preference $\mathcal{P}_u$ in the conversation, and $\widehat{\mathcal{V}}_{u}^-$ is the subset of $\mathcal{V}_{cand}$ that excludes the observed items $\mathcal{V}_{u}^{+}$. The two types of pairwise training instances is defined as:
\begin{equation}
    \mathcal{D}_1 := \{(u, v, v') \mid v' \in \mathcal{V}_{u}^- \}, \quad \mathcal{D}_2 := \{(u, v, v') \mid v' \in \widehat{\mathcal{V}}_{u}^- \},
\end{equation}

We then train the FM model by optimizing
%the instances in
both $\mathcal{D}_1$ and $\mathcal{D}_2$:
\begin{equation}
%\vspace{-10pt}
\begin{aligned}
    L_{item} &= \sum_{(u,v,v')\in \mathcal{D}_1} -\mbox{ln} \sigma(\hat{y}(u,v,\mathcal{P}_u) - \hat{y}(u,v',\mathcal{P}_u)) \\
    &+ \sum_{(u,v,v')\in \mathcal{D}_2} -\mbox{ln} \sigma(\hat{y}(u,v,\mathcal{P}_u) - \hat{y}(u,v',\mathcal{P}_u)) + \lambda_{\Theta} \left\|\Theta\right\|^2,
\end{aligned}
%\vspace{-3pt}
\end{equation}
where the first loss learns $u$'s general preference, and the second loss learns $u$'s specific preference given the current candidates. It is worth noting adding the second loss for training is critical for the model ranking well on the current candidates. This is very important for CRS since the candidate items dynamically change with user feedback along the conversation. However, the state-of-the-art method CRM~\cite{Sun:2018:CRS:3209978.3210002} does not account for this factor, being insufficient in considering the interaction between the CC and RC.

\subsubsection{Attribute Preference Prediction.} We formulate the task of the second goal of accurate attribute prediction separately. This prediction of attribute preference is mainly used in the CC to support the action on which attribute to ask ({\it c.f.} Sec~\ref{ss:action}). As such, we take $u$'s preferred attributes in the current session into account:
%Given a user $u$, and a set of known preference attributes $\mathcal{P}_{u}$, We use a similarity based method to predict unknown preference attributes $\mathcal{P} \backslash \mathcal{P}_{u}$, specifically we use cosine similarity between unknown attribute embedding and known attribute embedding with user embedding.
\begin{equation}\label{eq:sim}
    \hat{g}(p|u,\mathcal{P}_u) = \textbf{u}^T \textbf{p} + \sum_{p_i\in \mathcal{P}_u} \textbf{p}^T \textbf{p}_i,
    % \vspace{-5pt}
\end{equation}
which estimates $u$'s preference on attribute $p$, given $u$'s current preferred attributes $\mathcal{P}_u$.
To train the model, we also employ BPR loss, and assume that the attributes of the ground truth item $v$ (of the session) should be ranked higher than other attributes:
%is an unknown attribute.%, and \textbf{bold} means the hidden embedding vector.
%In light of this, we designed the pairwise loss for optimizing feature similarity.
%Given a user $u$, a item $v_{i}$, its attributes $\mathcal{P}_{i}$, and currently known attribute $\mathcal{P}_{u}$, the positive attributes are $\mathcal{P}_{i} \backslash \mathcal{P}_{u}$, the negative attributes are randomly chosen from $\mathcal{P} \backslash \mathcal{P}_{i}$
\begin{equation}
% \vspace{-8pt}
\begin{aligned}
    L_{attr} = \sum_{(u,p,p')\in \mathcal{D}_3} -\mbox{ln} \sigma(\hat{g}(p|u, \mathcal{P}_u) - \hat{g}(p'|u, \mathcal{P}_u)) + \lambda_{\Theta} \left\|\Theta\right\|^2,
\end{aligned}
\end{equation}
where the pairwise training data $D_3$ is defined as:
\begin{equation}
    D_3 = \{(u, p, p')| p\in \mathcal{P}_v, p'\in \mathcal{P} \backslash \mathcal{P}_v \},
    % \vspace{-4pt}
\end{equation}
where $\mathcal{P}_v$ denotes item $v$'s attributes.

\subsubsection{Multi-task Training.}\label{ss:multi-task}
We perform joint training on the two tasks of item prediction and attribute prediction, which has the potential of mutual benefits since their parameters are shared. The multi-task training objective is:
\begin{equation}
    % \vspace{-5pt}
    L = L_{item} + L_{attr}.
\end{equation}

\noindent Specifically, we first train the model with $L_{item}$. After it converges, we continue optimizing the model using $L_{attr}$. We iterate the two steps until convergence under both losses.  Empirically, 2-3 iterations are sufficient for convergence.

\subsection{Action}\label{ss:action}

%The task of recommendation also brings new challenges to conversation system: the CRS needs to hit the user preferred items within less turns. This requires a CC to be aware of the user dynamic preference when choosing a dialogue action. Therefore,

After the estimation stage, the action stage finds the best strategy for \textit{when to recommend}. We adopt reinforcement learning (RL) to tackle this multi-round decision making problem, aiming to accomplish successful recommendation in shorter number of turns.
% In the \emp{action} stage, the CC component in our EAR strategically chooses an action in order to make a successful recommendation within fewer turns. It is straightforward to model such decision making process as a reinforcement learning problem as has been practiced in many existing dialogue systems~\cite{acl18/sequicity,sigir18/chatmore,DRL4DG}. However, our action choosing process serves for the recommendation goal, which requires each action to be carefully decided based on the RS.
% For example, the CC needs to ask about an attribute that eliminates the uncertainty of user preference estimation for the RS, meanwhile, avoids asking attributes that a user is unlikely to prefer. This motivates the CC component to exploit the
% %where a dialogue policy network makes decisions based on
% statistics from the RC component to make the decision.
% Previous
% It is worth noting that since our focus is on the conversational recommendation strategy, rather than
% the language part, we leave out the understanding of user utterances and response generation.
% That is to say, all user utterances and system responses are generated by templates.
% %$Note that, all utterances are using template in this work. This means our CC only focus on dialogue action choice without handling the utterance understanding and response generation.
% Without error propagation from the utterance understanding and generation, this research can be treated as providing an upper bound study of real applications. In practice, we can leverage on any existing dialogue system as a wrapper to handle the language part.
%Now
% Yisong: Is it better to place in the dataset part?
It is worth noting that since our focus is on conversational recommendation strategy, as opposed to fluent dialogue (the language part), we use templates as wrappers to handle user utterances and system response generation.
% Min BUG: what do you mean by "upper bound" here?  I don't follow
% Wenqiang: addressed by adding an explanation.
That is to say, this work serves as an upper bound study of real applications as we do not include the errors for language understanding and generation. %In practice, we can leverage on any existing dialogue system as a wrapper to handle the language part.

\subsubsection{State Vector.} The state vector is a bridge for the interaction between the CC and RC. We encode information from the RC and dialogue history into a state vector, providing it to the CC to choose actions.
The state vector is a concatenation of four component vectors that encode signal from different perspectives:

\vspace{-10pt}
\begin{equation}\label{eq:state}
    \textbf{s} = \textbf{s}_{ent} \oplus \textbf{s}_{pre} \oplus \textbf{s}_{his} \oplus \textbf{s}_{len}.
\end{equation}

Each of the vector components captures an assumption on asking which attribute could be most useful, or whether now is a good time to push a recommendation. They are defined as follows:
\begin{itemize}[leftmargin=1mm]
    \item $\textbf{s}_{ent}$: This vector encodes the entropy information of each attribute among the attributes of the current candidate items $\mathcal{V}_{cand}$. The intuition is that asking attributes with large entropy helps to reduce the candidate space, thus benefits finding desired items in fewer turns. Its size is the attribute space size $|\mathcal{P}|$, where the $i$-th dimension denotes the entropy of the attribute $p_i$.
    %An entropy vector where the $i-th$ dimension is the entropy of attribute $P_{i}$ in the current candidate. If the preference of an attribute has been asked before, the corresponding dimension is set to be $0$. This vector encodes the uncertainty of each attribute in the candidate list. Asking a feature with max entropy has proven be a efficient strategy~\cite{}.
    \item $\textbf{s}_{pre}$: This vector encodes $u$'s preference on each attribute. It is also of size $|\mathcal{P}|$, where each dimension is evaluated by Equation~(\ref{eq:sim}) on the corresponding attribute. The intuition is that the attribute with high predicted preference is likely to receive positive feedback, which also helps to reduce the candidate space.
    %If an attribute has been asked before, we set the corresponding dimension as 0 to avoid asking it again.
    %A similarity vector where each dimension is the normalized similarity score calculated in given $u$ and $\mathcal{P}_{u}$.
    %If the preference of an attribute has been asked before, the corresponding dimension is set to be $0$. This encodes the estimated user preference towards an attribute. Asking a feature with high similarity make sure the model get useful feedback.
    \item $\textbf{s}_{his}$: This vector encodes the conversation history. Its size is the number of maximum turns $T$, where each dimension $t$ encodes user feedback at turn $t$. Specifically, we use -1 to represent recommendation failure, 0 to represent asking an attribute that $u$ disprefers, and 1 to represent successfully asking about an attribute that $u$ desires. This state is useful to determine when to recommend items. For example, if the system has asked about a number of attributes for which $u$ approves, it may be a good time to recommend.
    \item $\textbf{s}_{len}$: This vector encodes the length of the current candidate list. The intuition is that if the candidate list is short enough, EAR should turn to recommending to avoid wasting more turns. We divide the length $|\mathcal{V}_{cand}|$ into ten categorical (binary) features to facilitate the RL training.   %Instead of directly using $|\mathcal{V}_c|$, we discrete it into ten
    %The only contains one dimension which records the length of the current candidate list. The intuition is that if a candidate list is short enough, a better action is to make a recommendation.
\end{itemize}

\noindent It is worth noting that besides $\textbf{s}_{his}$, the other three vectors are all derived from the RC component.
We claim that this is a key difference from existing conversational systems~\cite{zhang2018towards,nips18/DeepConv,Sun:2018:CRS:3209978.3210002,christakopoulou2018q,Liao:2018}; i.e., the CC needs to take information from the RC to decide the dialogue action. In contrast to EAR, the recent conversational recommendation method CRM~\cite{Sun:2018:CRS:3209978.3210002} makes decisions based only on the belief tracker that records the preferred attributes of the user, which makes it less informative. As such, CRM is less effective especially when the number of attributes is large (their experiments only deal with 5 attributes, which is insufficient for real-world applications).

\subsubsection{Policy Network and Rewards} The conversation action is chosen by a policy network in our CC. In order to demonstrate the efficacy of our designed state vector, we purposely choose a simple policy network --- a two-layer multi-layer perceptron, which can be optimized with the standard policy gradient method.
It contains two fully-connected layers
% that are activated by the $tanh$ function
and maps the state vector $\textbf{s}$ into the action space. The output layer is normalized to be a probability distribution over all actions by $softmax$.
%Intuitively, the agent will take many factors into account to decide which action to take at each turn, e.g. current candidate item space, user feedback in previous turns, information about unknown attributes, as these factors can be vectorized, it is very fitting for us to use a deep reinforcement learning to model and optimize such decision behavior.
In terms of the action space, we follow the previous method \cite{Sun:2018:CRS:3209978.3210002}, which includes all attributes $\mathcal{P}$ and a dedicated action for recommendation. To be specific, we define the action space as $\mathcal{A} = \{ a_{rec} \cup \{ a_{ask}(p) | p\in \mathcal{P}\} \},$
% \begin{equation}
%     \mathcal{A} = \{ a_{rec} \cup \{ a_{ask}(p) | p\in \mathcal{P}\} \},
% \end{equation}
which is of size $|\mathcal{P}|+1$.
After the CC takes an action at each turn, it will receive an immediate reward from the user (or user simulator).
This will guide the CC to learn the optimal policy that optimizes long-term reward. In EAR, we design four kinds of rewards, namely: (1) $r_{suc}$, a strongly positive reward when the recommendation is successful, (2) $r_{ask}$, a positive reward when the user gives positive feedback on the asked attribute, (3) $r_{quit}$, a strongly negative reward if the user quits the conversation, (4) $r_{prev}$, a slightly negative reward on every turn to discourage overly lengthy conversations.
% \begin{itemize}[leftmargin=*]
%     \item $r_{suc}$, a strongly positive reward when the recommendation is successful.
%     \item $r_{ask}$, a positive reward when the user gives positive feedback on the asked attribute.
%     \item $r_{quit}$, a strongly negative reward if the user quits the conversation.
%     \item $r_{prev}$, a slightly negative reward on every turn to discourage the conversation goes too long.
% \end{itemize}
The intermediate reward $r_t$ at turn $t$ is the sum of the above four rewards, $r_t=r_{suc}+r_{ask}+r_{quit}+r_{prev}$.
% namely:
% \begin{equation}
%     r_t=r_{suc}+r_{ask}+r_{quit}+r_{prev}
% \end{equation}

We denote the policy network as $\pi(a^t\mid\textbf{s}^t)$, which returns the probability of taking action $a^t$ given the state $\textbf{s}^t$. Here $a^t\in \mathcal{A}$ and $\textbf{s}^t$ denote the action to take and the state vector of the $t$-th turn, respectively.
%we denote the probability of taking action $a_{i}$ given state $s_{i}$ at step $i$ as $\pi(a_{i}$\mid$s_{i}$), and
To optimize the policy network, we use the standard policy gradient method~\cite{REINFORCE}, formulated as follows:
%REINFORCE~\cite{REINFORCE} algorithm, which updates after one episodes terminates by calculating the cumulative reward at each step, and directly update the policy's weight by:
 \begin{equation}
    \theta \leftarrow \theta - \alpha \bigtriangledown \mbox{log} \pi_{\theta}(a^t\mid \textbf{s}^t) R_{t},
\end{equation}
where $\theta$ denotes the parameter of the policy network, $\alpha$ denotes the learning rate of the policy network, and $R_{t}$ is the total reward accumulating from turn $t$ to the final turn $T$: $R_t = \sum_{t'=t}^{T} \gamma^{T-t'}r_{t'},$
% \begin{equation}
%     R_t = \sum_{t'=t}^{T} \gamma^{T-t'}r_{t'},
% \end{equation}
where $\gamma$ is a discount factor which discounts future rewards over immediate reward.

\subsection{Reflection}
This stage also implements the interaction between the CC and RC. It is triggered when the CC pushes the recommended items $\mathcal{V}^{t}$ to the user but gets rejected, so as to update the RC model for better recommendations in future turns.
%In a conversational recommendation scenario, the CC component helps the RC component to dynamically get feedbacks. What we have discussed before are feedbacks of the user explicit preference towards an item. However, it is possible to infer the implicit preference from the user rejection items.
In the traditional static recommender system training scenario~\cite{BPR,NCF}, one issue is the absence of true negative samples, since users do not explicitly indicate what they dislike.
In our conversational case, the rejection feedback is an explicit signal on user dislikes which are highly valuable to utilize; moreover, it indicates that the offline learned FM model improperly assigns high scores to the rejected items.
To leverage on this source of feedback, we treat the rejected items $\mathcal{V}^{t}$ as negative samples, constructing more training examples to refresh the FM model. Following the offline training process, we also optimize the BPR loss:
%e can regulate the learned preference by constructing negative training examples using the rejected items. Following the offline training process, we also adopt BPR loss to update our RS.  Formally, we treat the $\mathcal{V^{t}}$ as a set of negative samples and use the positive samples from training set to mini-batch update the RC model. This process is mathematically formulated as follows:
% \vspace{-3pt}
\begin{equation}
    L_{ref} = \sum_{(u,v,v')\in \mathcal{D}_4} -\mbox{ln} \sigma(\hat{y}(u,v,\mathcal{P}_u) - \hat{y}(u,v',\mathcal{P}_u)) + \lambda_{\Theta} \left\|\Theta\right\|^2
% \vspace{-5pt}
\end{equation}
where $\mathcal{D}_4 := \{(u, v, v') \mid v \in \mathcal{V}_{u}^{+} \wedge v' \in \mathcal{V}^{t}\}$. Note that this stage is performed in an online fashion, where we do not have access to the ground truth positive item. Thus, we treat the historically interacted items $\mathcal{V}^+_u$ as the positive items to pair with the rejected items. We put all examples in $D_4$ into a batch and perform batch gradient descent. Empirically, it takes 3-5 epochs to converge, sufficiently efficient for online use.

Note that although it sounds reasonable to also update the policy network of the CC (since the rejection feedback implies that it is not an appropriate timing to push recommendation), we currently do not perform this due to high difficulty of online updating RL agent and leave it for future work. %How to appropriately update the reinforcement learning agent online is left as future work.

% . However, it is highly complicated to update the
% Many previous research~\cite{} has shown the efficacy of online updating recommendation models.
% However, we need to figure out it is a complex research direction itself.
% It is a complex research problem. So we do not discuss much. we only explore a simple one which has been demonstrated effective.


==> ear-arxiv-new/Preliminary.tex <==
\section{Multi-round Conversational Recommendation Scenario}\label{sec:pre}

% distinguish multi-turn and multi-round
%This paper considers a \textit{multi-round} conversational recommendation scenario, where a CRS interacts with the user by asking attributes and recommending items multiple times until task success or the user leaves. This is more sophisticated yet realistic than  previous settings~\cite{Sun:2018:CRS:3209978.3210002}, in which the CRS only makes recommendations once and ends the session regardless of success or not. Here, we denote one trial of recommendation as a \emph{round}, following the terminology introduced in \cite{christakopoulou2018q}. To distinguish our scenario with the settings that only recommend items once (i.e., single-round)~\cite{Sun:2018:CRS:3209978.3210002,christakopoulou2018q}, we refer to our scenario as multi-round conversational recommendation. Next, we introduce the necessary mathematical notations to describe the scenario that are used across the paper.  

\begin{figure}[t]
\centering
%\includegraphics[width=\columnwidth,height=3cm]{model-picture-edit-4.pdf}\vspace{-5pt}
\includegraphics[height=5cm]{model-picture-edit-4.png}\vspace{-10pt}
\caption{The workflow of our multi-round conversational recommendation scenario. The system may recommend items multiple times, and the conversation ends only if the user accepts the recommendation or chooses to quit.}\vspace{-10pt}
\label{fig:preli_workfolow}
\vspace{-10pt}
\end{figure}


Following~\cite{christakopoulou2018q}, we denote one trial of recommendation as a \emph{round}. This paper considers conversational recommendation as an inherently \textit{multi-round} scenario, where a CRS interacts with the user by asking attributes and recommending items multiple times until the task succeeds or the user leaves. To distinguish the two, we term the setting \emph{single-round} where the CRS only makes recommendations once, ending the session regardless of the outcome, as in \cite{Sun:2018:CRS:3209978.3210002,christakopoulou2018q}. 

%Assume EAR is recommending items $v$ for users $u$. $v$ can be any items for recommendation. In the current work, an artist in the LastFM dataset and a restaurant in the Yelp dataset is treated an item accordingly. Each item can have one or multiple attribute $P$. For example, an artist might have attributes like {\tt classic} or {\tt jazz} and a business has its business type like {\tt nightlife}, {\tt serving burgers} and {\tt serving wines} etc.
We now introduce the notation used to formalize our setting.
Let $u\in\mathcal{U}$ denote a user $u$ from the user set $\mathcal{U}$ and $v\in\mathcal{V}$ denote an item $v$ from the item set $\mathcal{V}$. Each item $v$ is associated with a set of attributes $\mathcal{P}_v$ which describe its properties, such as music genre ``classical'' or ``jazz'' for songs in LastFM, or tags such as ``nightlife'', ``serving burgers'', or ``serving wines'' for businesses in Yelp. We denote the set of all attributes as $\mathcal{P}$ and use $p$ to denote a specific attribute. 
Following~\cite{Sun:2018:CRS:3209978.3210002,zhang2018towards}, a CRS session is started with $u$'s specification of a preferred attribute $p^0$,
%After obtaining initial preferences, 
then the CRS filters out candidate items that contain the preferred attribute $p^0$.
Then in each turn $t$ ($t=1, 2, ..., T$; $T$ denotes the last turn of the session), the CRS needs to choose an action: \textit{recommend} or \textit{ask}:
\begin{itemize}[leftmargin=*]
% Min: the actions should be formatted to stand out from the sentences' normal words.
% Yisong: done
    \item If the \textsc{action} is \emph{recommend}, we denote the recommended item list $\mathcal{V}^t\subset\mathcal{V}$ and the action as $a_{rec}$. Then the user examines whether $\mathcal{V}^t$ contains his desired item. If the feedback is positive, this session succeeds and can be terminated. Otherwise, we mark $\mathcal{V}^t$ as \textit{rejected} and move to the next round.
    \item If the \textsc{action} is \emph{ask} (where the asked attribute is denoted as $p^t\in\mathcal{P}$ and the action as $a_{ask}(p^t)$), the user states whether he prefers items that contain the attribute $p^t$ or not. If the feedback is positive, we add $p^t$ into $\mathcal{P}_u$ to denote the preferred attributes the user in the current session. Otherwise, we mark $p^t$ as \textit{rejected}; regardless of rejection or not, we move to the next turn. 
\end{itemize}

%If it feels confident about the user preference, it recommends a list of items to the user; . Otherwise, it asks an attribute to solicit more explicit information about user preference; we denote the asked attribute as . 

%The user responds to the CRS according to his current preference $P_{all}$, (1) for CRS asking an attribute $P_{k}$, the user will examine if $P_{k}$ is within $P_{all}$, and response YES or NO (2) for CRS proposing a list of recommendation, the user will examine if the list of item contains his desired item(s). 

%If a CRS decides to attribute $P_{k}$ to reduce uncertainty, a user respond it by indicating whether he/she likes the attribute or not. The CRS will take this attribute feedback to choose another action. If the CRS is confident and proposes RecList to the user,  he/she examines whether the list of item contains his desired item(s). In case none of the item in the RecList is preferred by the user, he will reject this recommendation. As a result, the RecList will be RejList which is also treated as feedback for the CRS to make a new chooise a new action. It is possible to continue to recommend another list of items immediately after a rejection feedback. This scenario is also more realistic than the SAUR paradigm~\cite{zhang2018towards} where a system is only designed to ask questions after a rejecting feedback. Our scenario gives more flexibility as well as challenges to a dialogue system.  

%Table~\ref{tab:glossary} summarizes the notations used in this paper including the ones to be introduced in method. 
\noindent 
%All notations can found in Table~\ref{tab:glossary} and the whole process is demonstrated in Figure~\ref{fig:preli_workfolow}. 
This whole process naturally forms a interaction loop (Figure~\ref{fig:preli_workfolow}) where the CRS may ask zero to many questions before making recommendations. 
A session terminates if a user accepts the recommendations or leaves due to his impatience.  We set the main goal of the CRS as making desired recommendations within as few rounds as possible. 


%To addresss it, we decompose this challenge into three fundamental problems as discussed in Section XXX: 1) What questions to ask regarding item attributes? 2) When to recommend items? 3) How to adapt to user online feedback?


%We refer to a loop of series actions as a \emph{round}. Formally, a round is defined using a regular expression:
%\begin{equation}
%    round=[asking a question]-->make recommendation
%\end{equation}
 

%Assume EAR is recommending items $v$ for users $u$. $v$ can be any items for recommendation. In the current work, an artist in the LastFM dataset and a restaurant in the Yelp dataset is treated an item accordingly. Each item can have one or multiple attribute $P$. For example, an artist might have attributes like {\tt classic} or {\tt jazz} and a business has its business type like {\tt nightlife}, {\tt serving burgers} and {\tt serving wines} etc. %Those attributes are tags given by their users. 

%%%Wenqiang: 给一个mathematical formulation。说我们这个问题要在轮数少的情况下准确率尽可能地高。
%然后这里就formalize出三个问题。 
% user只能选我们给定的attribute。 
%Each conversation session is started by a user informing an attribute $P_{0}$ to the CRS, the CRS can conduct two kinds of actions, (1) $a_{ask}_{i}$: asking i--th attribute $P_{i}$ from the whole attribute space \mathcal{P}, and (2) $a_{rec}$: proposing a recommendation list to the user.
%The user responds to the CRS according to his current preference $P_{all}$, (1) for CRS asking an attribute $P_{k}$, the user will examine if $P_{k}$ is within $P_{all}$, and response YES or NO (2) for CRS proposing a list of recommendation, the user will examine if the list of item contains his desired item(s). \par

%So we can see, as the turn of the conversation increases, the CRS gradually accumulated two types of information: (1) it has confirmed a set of attributes from user, e.g. \{$P_{0}$, $P_{6}$, $P{17}$\}(we denote such known preference set by $P_{K}$), so it can narrow down the candidate item list(denoted by $CanList$) to those items containing all the attributes in $P_{K}$(2) when CRS propose recommendation to user, it might be rejected by the user, thus the CRS can also learn from previous failure recommendation list(denoted by $RejList$). \par

%In order to gain more evidence quickly to realize the goal that we successfully recommend user's desired item in shortest turns, we summarize three key fundamental problems as discussed in \textbf{Section 1}: 1) What questions to ask regarding item attributes? 2) When to recommend items? 3) How to adapt to user online feedback?

%We will discuss the solution to these three questions in next section.
%Ideally, a EAR need to runs in an online surrounding which is hard to be accessed by academia. As an alternative solution, we follow~\cite{Sun:2018:CRS:3209978.3210002} to build simulator on offline datasets to mimic the online environment. In our experiment, we choose two popular datasets -- namely, Yelp for XXX recommendation and lastFM for artist recommendation (\emph{c.f.} Sec.XXX) -- in traditional static recommendation settings. In such dataset, a user $u_i$ from the user set $notation$ have multiple visit records for a set of items $i notation$ (a business in Yelp dataset and an artists in lastFM dataset). Each item has multiple attributes. For example, an artist might have attributes like {\tt classic} or {\tt jazz} and a business has its business type like {\tt nightlife}, {\tt serving burgers}. Those attributes are tags given by their users. 


% We split all the visit record into training, validation and testing sets according to XXXX. In the testing and validation set, a user simulator is understand 



%Assume EAR is running on a system to recommend item to user conversationally, in our current work, the item can be an artist (in the LastFM dataset) or a business (in the Yelp dataset). Each item has multiple attributes, the attribute can be music type like classic or jazz for lastFM dataset / business type like nightlife, burgers or Japanese for yelp dataset. When a user tagged or reviewed an item, we consider he/she likes this item and treats it as positive samples. 


%\begin{table}[t]
%\caption{Key notations.}\small\label{-5pt}
%\label{tab:glossary}
%%\begin{tabular}{|l{2cm}|l{4cm}|}
%\begin{tabular}{|m{1.5cm}|m{6cm}|}
%\hline
%$u,v,p$;  & a user, an item, an attribute  \\ \hline
%$\mathcal{U},\mathcal{V},\mathcal{P}$; & all users, all items, all attributes \\ \hline
%$\mathcal{V}_{u}^{+}$ & items interacted by $u$ \\ \hline
%%$\mathcal{V}_{u}^{-}$ & the set of items user u has not interacted before \\ \hline
%%$\mathcal{P}$ & the whole attribute space \\ \hline
%$\mathcal{P}_{v}$ & attributes of item $v$ \\ \hline
%$\mathcal{P}_{u}$ & attributes preferred by user $u$ in a conversation \\ \hline
%$\mathcal{V}_{cand}$ & candidate items that satisfy attributes in $\mathcal{P}_{u}$ \\ \hline
%$p^m$ & the \textit{m}--th attribute in attribute space \\ \hline
%$p^0$ &  user's initial indication on one attribute \\ \hline
%T & max turn of conversation \\ \hline
%$v_{target}$& the target item in a conversation session \\ \hline
%$a_{k}$ A & the action at k--th turn and the whole action space \\ \hline
%$a_{ask}(p^t)$ & the action of asking p--th attribute \\ \hline
%$a_{rec}$ & the action of making recommendation of item set $\mathcal{V}^t$ \\ \hline
%%$InterHis$ & \makecell{Interaction history in current conversation session\\ containing CRS's action and user's response}  \\ \hline
%% &  \\ \hline
%\end{tabular}
%\end{table}

%\begin{figure}[t]
%\centering
% Min: Terrible space use.  Reformat for horizontal aspect ratio.  Use a better text font size to rectangular area. 
%\includegraphics[scale=0.3]{model-picture-2.pdf}
%\caption{The structure of EAR model}
%\label{fig:overview}
%\end{figure}

==> ear-arxiv-new/Rela.tex <==
% Below are new relavent works:
% Yisong: Relevant Work 1
% https://arxiv.org/pdf/1906.01219  Bandit for conversational recommendation.  李航
% Different from other bandit method that can only push recommendation, their system can also ask questions for attributes. However, we formalize the problem from totally different angle, i.e. we focus on the interaction between CS and RS, but they treat the asking attribute as `key-term selection` and formalize it under bandit framework (many math, regret analysis). 
% They haven't published yet, only on Arxiv. Do we need to cite them? I guess it's CIKM, camera ready is Aug 27.
% Wenqiang: bandit can recommend one item each time. I guess this is a key difference.


% Yisong: Relavant Work 2
% https://arxiv.org/pdf/1907.00710.pdf Deep Conversational Recommender in Travel. Lizi Liao
% Submitted to TKDE, haven't accepted yet.
% Main focus are: (1) topic control, (2) use GCN to recommend (match between venue and dialog context); (3) pointer network for response generation.
% They lack: didn't emphasize the strategy.
% Wenqiang: I guess this paper is more like to be a dialogue system, like the NIPS 2018 paper.

% Relavent Work 3 
% An Visual Dialog Augmented Interactive Recommender System. KDD 2019
% A short video: https://www.youtube.com/watch?v=GvgBgwGsWcM&feature=youtu.be
% webpage: https://www.kdd.org/kdd2019/accepted-papers/view/an-visual-dialog-augmented-interactive-recommender-system
% The input data in each rounds include: a list of item with user feedback(click / comment), they model user viewing, clicking, commenting
% Key difference: their system cannot explicitly ask user for an attribute, and user have to (click / write comment) on a few items at each rounds.

% Related Work 4
% Ontology-based conversational recommender system for recommending laptop https://iopscience.iop.org/article/10.1088/1742-6596/1192/1/012020/pdf  
% It is on a Physics Journal, do we need to cite it?
% Wenqiang: Yes.

% Related Work 5
% An Approach to Conversational Recommendation of Restaurants. https://link.springer.com/chapter/10.1007/978-3-030-23525-3_16
% Cannot download paper, and the abstract is too generic.

% Related Work 6
% Preference Elicitation Strategy for Conversational Recommender System. WSDM2019, 2 page paper.
% Only focus on how to ask feature, rather than the strategy to recommend.

\section{Related Work}\label{sec:related}
The offline \textbf{static recommendation} task is formulated as estimating the affinity score between a user and an item~\cite{NCF}. This is usually achieved by learning user preferences through the historical user-item interactions such as clicking and purchasing. The representative methods are Matrix Factorization (MF)~\cite{MF} and Factorization Machine (FM)~\cite{rendle2010factorization}. Neural FM~\cite{NFM} and DeepFM~\cite{guo2017deepfm} have improved FM's representation ability with deep neural networks. \cite{fastMF,iCD,sigir/EbesuSF18} utilize user's implicit feedback, commonly optimizing BPR loss~\cite{BPR}. \cite{cheng2019mmalfm, cheng2018aspect} exploits user's reviews and image information.  However, such static recommendation methods suffer from the intrinsic limitation of not being able to capture user dynamic preferences.

This intrinsic limitation motivates \textbf{online recommendation}. Its target is to adapt the recommendation results with the user's online actions~\cite{li2015online}. Many model it as a multi-arm bandit problem
% ~\cite{kuleshov2014algorithms,auer2002finite,li2016collaborative,gentile2016context,wu2016contextual,wang2017factorization,wu2018learning,cikm13/ICF}
~\cite{wu2016contextual,wang2017factorization,wu2018learning}
, strategically demonstrating items to users for useful feedback. \cite{zhang2019toward} makes the preliminary effort to extend the bandit framework to query attributes. While achieving remarkable progress, the bandit-based solutions are still insufficient: 1) Such methods focus on exploration--exploitation trade-off in cold start settings. However, in warm start scenario, capturing the user dynamic preference is critical as preference drift is common; 2) The mathematical formation of multi-arm bandit problem limits such method only recommend one item each time. This constraint limits its application, as we usually need to recommend a list of items.

\textbf{Conversational recommender systems} provide a new possibility for capturing dynamic feedback as they enable a system to interact with users using natural language. However, they also pose challenges to researchers, leading to various settings and problem formulations ~\cite{christakopoulou2016towards,nips18/DeepConv,Liao:2018, christakopoulou2018q,zhang2018towards,Sun:2018:CRS:3209978.3210002, priyogi2019preference, liao2019deep, yu2019visual, ayundhita2019ontology, sardella2019approach, zhang2019toward}. Table~\ref{tab:CRS}  summarizes these works' key aspects. Generally, prior work considers conversational recommendation only under simplified settings. For example, \cite{christakopoulou2016towards, yu2019visual} only allow the CRS to recommend items without asking the user about their preferred attributes. The Q\&R work~\cite{christakopoulou2018q} proposes to jointly optimize the two tasks of attribute and item prediction, but restricts the whole conversation to two turns: one turn for asking, one turn for  recommending.  CRM~\cite{Sun:2018:CRS:3209978.3210002} extends the conversation to multi-turns but still follows the single-round setting. MMN~\cite{zhang2018towards} focuses on document representation, aiming to learn better matching function for attributes and products description under a conversation setting. Unfortunately, it does not build a dialogue policy to decide when to ask or make recommendations. 
In contrast, situations for various real applications are complex: the CRS needs to strategically ask attributes and make recommendations in multiple rounds, achieving successful recommendations in the fewest turns. In recent work, only~\cite{nips18/DeepConv} considers this multi-round scenario, but it focuses on language understanding and generation, without attending to explicitly model the conversational strategy.

% Min: repetitive -- omit
% Different from existing works, we focus on dialogue strategy in the multi-round recommendation scenario and design a model based on the ideology that CC and RC, the two essential components, need to achieve deep interactions. To the best of our knowledge, we are the first to systematically model such interactions. 
% \vspace{-10pt}

%To summarize, existing conversational recommender systems either ignore the strategy for when to recommend or only consider single-round conversation that recommends items once. 
%We are the first that focuses on the most essential elements of building CRS --- deep interaction between CS and RS. 

%To achieve that, we hypothesize the CC and RC need to closely interact or support each other.



%We briefly review related work of traditional offline recommendation and online conversational recommendation. 

%\subsection{Traditional Static Recommendation}
%The offline recommendation task is formulated as estimating the affinity score between a user and an item~\cite{NCF}. 
%SPACE
%This is usually achieved by leveraging historical user-item interactions, which can be divided into explicit or implicit, according to whether users have explicitly expressed like/dislike preference. 
%Early recommendation work has largely focused on explicit feedback, i.e., predicting the rating scores~\cite{adomavicius2005toward,MF}. As implicit feedback is much easier to obtain with a much lower cost~\cite{BPR} (e.g., serve logs on clicks and purchases), 

%Existing static offline recommendation system has demonstrated a great success to facilitate users seeking information [].  It ...
%However, as discussed in Section~\ref{sec:introduction}, the traditional recommendation suffers from the intrinsic limitations in precisely capture user dynamic preference. This work is towards this problem by introducing a conversational recommendation system. It is a integration a conversational component (CC) and a recommendation component (RC). By such integration, we can 



%next generation of recommender systems to be able to dynamically obtain user preference when doing recommendation.


%, which can be divided into explicit or implicit, according to whether users have explicitly expressed like/dislike preference.  

%Recent research on building offline recommender models has shifted from explicit feedback~\cite{MF} to implicit feedback~\cite{fastMF,iCD,sigir/EbesuSF18}.
%One key difference
%in learning from the one-class implicit data
%is in the objective function, such that the negative feedback need to be modeled from the unobserved missing data~\cite{iCD,hu2008collaborative}.
%One common way is to optimize models with pairwise loss between observed and sampled missing data, as advocated by the BPR work~\cite{BPR}. It has been shown that the quality of negative samples plays a critical role on model performance, e.g., large improvements by sampling hard negatives~\cite{DNS} or trustful negatives~(e.g., viewed but not purchase)~\cite{ding2018improved}. 
%In this work, we build offline recommender models by assuming the feedback is implicit, and uses BPR as the objective function. 
%In this work, we adapt the training process of BPR
%to tailor it for learning from conversation logs, especially taking user preferred attributes in each turn into account to find more informative negative samples. This substantially improves model performance and to our knowledge, has never been explored before. 

%In terms of offline predictive models, some representative achievements include Matrix Factorization (MF)~\cite{MF} which learns latent features (a.k.a., embedding) for users and items, Factorization Machine (FM)~\cite{rendle2010factorization} which applies the idea of factorization to model any side information, %Collaborative Deep Learning (CDL)~\cite{CDL} which enriches item embeddings with deep representations from affiliated texts,
%Neural Collaborative Filtering (NCF)~\cite{NCF} which learns the user-item interaction function with expressive neural networks, 
%and Neural FM~\cite{NFM} and DeepFM~\cite{guo2017deepfm} that improve FM representation ability with deep neural networks. 
%In this work, we choose FM as the offline recommender model, due to its ease and interpretability. 
%in integrating side information, like item attributes and user profiles (e.g., the preferred attributes during conversation). 
%We enhance FM by performing multi-task training on both tasks of item and attribute preference prediction. Though simple, this enhancement is important for the interaction between RC and CC --- a valuable signal for CC to make decisions on what attribute questions to ask. 

%Although much research effort has been devoted to offline recommendation methods, their inherent limitations cannot be ignored. First, optimizing the offline performance may not conform with the online testing metric. Second, a user keeps interacting with the system to seek desired information. It is important for the RC to take such online dynamics into account. This rises the need to develop methods for online recommendation. 

%\vspace{-5pt}
%\subsection{Online Recommendation}




%Much research has been conducted to address the exploration-exploitation trade-off in item selection~\cite{cikm13/ICF} by modeling it as a multi-arm bandit problem~\cite{kuleshov2014algorithms,auer2002finite,li2016collaborative,gentile2016context,wu2016contextual,wang2017factorization,wu2018learning}. However, in the setting of multi-armed 
%, that is, whether to exploit the known interests of users (e.g., predicted by offline recommenders) or explore the new interests by selecting diverse items~.
%Multi-armed bandit is an effective method to address the problem, which continuously interacts with different arms (items) and optimizes the total reward. 
%Traditional bandit methods include $\epsilon$-greedy~\cite{kuleshov2014algorithms} and Upper Confidence Bound (UCB) algorithm~\cite{auer2002finite}.
%Collaborative filtering effects have been recently introduced into the bandit algorithm~ \cite{li2016collaborative,gentile2016context,wu2016contextual,wang2017factorization,wu2018learning}.
%, and some representative work includes collaborative
%Linear UCB~\cite{wu2016contextual}, and factorization UCB~\cite{wang2017factorization}, and bandit algorithm in dynamic environment~\cite{wu2018learning}.

%Another solution is to online update model parameters or inputs with user real-time interactions. For example, \cite{fastMF,DynamicMF} propose to efficiently update the parameters of MF to keep the recommendations with user new behaviors.
%, and \cite{iCD} refreshes the recommendation by updating the input features to FM to include the user new behaviors. 
%In this work, we opt for this solution rather than bandits, since it caters well with our choice of offline recommenders and does not introduce extra technical complexity.
% Yisong: can comment this for space use.
%Given user positive feedback on attributes, we revise the input by adding user preferred attributes; given user negative feedback on recommendations, we update user embedding to rank these rejected items lower. Both online strategies make FM effective to adapt user online behaviors.   

%\vspace{-5pt}
%\subsubsection{Conversational Recommendation}\label{sec:crs-related}
%This topic is tightly related to online recommendation since a user must converse with the system in an online environment. 
%The envisionment of \textbf{conversational recommender system} provides a new possibility for online recommendations. It enables a system to obtain more user feedback through chatting with users.
%However, it also poses challenges to academia researchers. As a result, the definitions or settings of different work vary a lot~\cite{christakopoulou2016towards,nips18/DeepConv,Liao:2018, christakopoulou2018q,zhang2018towards,Sun:2018:CRS:3209978.3210002, priyogi2019preference, liao2019deep, yu2019visual, ayundhita2019ontology, sardella2019approach, zhang2019toward}. In Table~\ref{tab:CRS}, we summarize five characteristics of these recent formally published conversational recommenders.
%: 1) whether to ask questions besides recommendation, 2) what is the question space, 3) is there an explicit strategy to determine the time of pushing recommendations, 4) is it multi-round conversation that recommends items multiple items, and 5) what is the main focus of the work. Next we briefly review these work. 
%The work \cite{christakopoulou2016towards} uses a bandit method for online item selection with exploration-exploitation trade-off, thus it does not ask questions and has no strategy on when to recommend items (same for other bandit-based online recommendation methods~\cite{wu2016contextual,wu2018learning}).
%The REDIAL method \cite{nips18/DeepConv} employs an end-to-end dialogue model structure to generate natural language questions and responses, and incorporates movie recommendations by generating movie names; thus such strategy of recommendation timing is implicit rather than explicit.  
%Similarly for the KMD method~\cite{Liao:2018}, which does end-to-end generation by incorporating product image. 
%Although both methods do multi-round recommendations, they cannot incorporate user negative feedback on recommended items due to the lack of explicit recommendation strategy. 


%or example, \cite{christakopoulou2016towards} proposes a bandit method for online item selection and also terms the work as conversational recommendation. Later, the authors~\cite{christakopoulou2018q} propose to ask questions about item attributes before making recommendation and jointly optimize the two tasks of attribute prediction and item prediction. However, this work only has one-round conversation that recommends items once. 


%\subsection{Conversational Recommendation System}
%The term \textit{Conversational Recommendation System} can not be largely found in literature,  here we list the representative works in a chronological order. 

%Mehmet H. G{\"o}ker et.al. \cite{goker2000personalized} did the pioneer work for conversational recommendation system.  They proposed a user adaptive conversational recommendation system in order to help users  decide on a destination, specifically a restaurant.They rigorously defined several dialogue operators for both user and system, and define how these operator update the query and user model alongside the interaction.

%Christakopoulou et.al. \cite{christakopoulou2016towards} proposed an agent using bandit learning and active learning as question selection strategy. But their agent has very limited action space, it can ask user for absolute or pairwise opinion for the given item, and consequently the user's action space is limited to give YES/NO answers. %which is far from the \textit{'conversational'} as the author claimed.

%Ikemoto et.al. \cite{ikemoto2018conversation} proposed a Chatbot to do interactive recommendations. They model item and user by feature, and the Chatbot will continuously ask user for her preference for one feature or one item, and update model based on user's feedback. But they only used hand-crafted question strategy, and have to manually adjust the threshold for recommending item. Also they didn't use user's profile to have a \textit{warmer-start} as Christakopoulou et.al. did in ~\cite{christakopoulou2016towards}.

%Sun et.al. \cite{Sun:2018:CRS:3209978.3210002} proposed a new framework based on deep reinforcement, but the system actually only asks about facet value, so it somehow reduced to an \textit{interactive facet search system}).Given this, it might be more natural for user to select the facet value by clicking on the screen, rather than type a natural language sentence? Also, the agent does not attempt to recommend items to user as we did, which sacrifice the collaborative effect among items.

%\subsection{Multi-armed Bandit Algorithm}
%\subsection{Deep / Reinforcement Learning in interactive Recommendation System} 
%Nowadays reinforcement learning are being used in recommendation systems.\par Yuan et.al. \cite{zheng2018drn} proposed a novel deep reinforcement learning framework for news recommendation with DBGD(Dueling Bandit Gradient Descent) method for the exploration of reinforcement learning. Zhao et.al. \cite{zhao2018deep} used deep reinforcement learning for page-wise recommendation system. Christakopoulou et.al. \cite{christakopoulou2018q} designed a framework for interactive recommendation using sequential neural model.


